Why distillation helps: a statistical perspective

Knowledge distillation is a technique for improving the performance of a simple "student" model by replacing its one-hot training labels with a distribution over labels obtained from a complex "teacher" model. While this simple approach has proven widely effective, a basic question remains unresolved: why does distillation help? In this paper, we present a statistical perspective on distillation which addresses this question, and provides a novel connection to extreme multiclass retrieval techniques. Our core observation is that the teacher seeks to estimate the underlying (Bayes) class-probability function. Building on this, we establish a fundamental bias-variance tradeoff in the student's objective: this quantifies how approximate knowledge of these class-probabilities can significantly aid learning. Finally, we show how distillation complements existing negative mining techniques for extreme multiclass retrieval, and propose a unified objective which combines these ideas.

==> Why distillation helps ICML 2020/abstract.tex <==
%
Knowledge distillation is a technique for improving the performance of a simple ``student'' model by replacing its one-hot training labels with a \emph{distribution} over labels obtained from a complex ``teacher'' model. Despite proving widely effective, a basic question remains unresolved: why does distillation help? In this paper, we present a statistical perspective on distillation which 
%addresses this 
provides one answer to this
question and suggests a novel application to multiclass retrieval.
Our core observation is that the teacher seeks to estimate the underlying (Bayes) class-probability function. Building on this,
we establish a fundamental \emph{bias-variance} tradeoff for the student: this quantifies how approximate knowledge of these class-probabilities can significantly aid learning. 
Finally,
we extend this statistical perspective to multiclass \emph{retrieval} settings,
and propose a \emph{double-distillation}
objective which
encourages a good ranking over labels.
We empirically validate our analysis, and demonstrate  the value of double-distillation for retrieval. 


==> Why distillation helps ICML 2020/analysis.tex <==
We now present a statistical perspective of distillation,
which gives insight into why it can aid generalisation.
Central to our perspective are two observations:
\begin{enumerate}[label=(\roman*),itemsep=0pt,topsep=0pt]
    \item the risk~\eqref{eqn:risk} we seek to minimise 
    inherently smooths labels by the \emph{class-probability distribution} $\Pr( y \mid x )$;
    
    \item a teacher's predictions provide an approximation to the class-probability distribution $\Pr( y \mid x )$,
    which can thus yield a better approximation to the risk~\eqref{eqn:risk}
    than one-hot labels.
    %the teacher's predictions can be seen as an approximation to this distribution.
\end{enumerate}
Building on these, we show how sufficiently accurate teacher approximations can improve student generalisation.


%
%\subsection{Bayes knows best: the value of class-probabilities}
\subsection{Bayes knows best: distilling class-probabilities}
\label{sec:bayes-distillation}

Our starting point is the following elementary observation: 
the underlying risk $R( f )$
for a predictor $f \colon \XCal \to \Real^L$ is %expressible as
\begin{align}
\label{eq:population_risk}
    R( f ) &= \E{\X}{ \E{\Y \mid \X}{ \ell( \Y, f( \X ) ) } } \nonumber \\
    &= \E{\X}{ \pStar( \X )^{\tup} \ell( f( \X ) ) },
\end{align}
where $\pStar( x ) \defEq \begin{bmatrix} \Pr( y \mid x ) \end{bmatrix}_{y \in [ L ]} \in \Delta_{\YCal \defEq [L]}$ is the \emph{Bayes class-probability distribution}.
Intuitively, $\Pr( y \mid x )$ inherently captures the suitability of label $y$ for instance $x$.
Thus, the risk involves drawing an instance $\X \sim \Pr( {\X} )$, and then computing the average loss of $f( \X )$ over all labels $y \in [ L ]$, 
weighted by their
%true class-probabilities.
Bayes probabilities $\Pr( y \mid x )$.
When $\pStar( x )$ is not concentrated on a single label,
% the distribution has \emph{nonzero Bayes error},
there is an \emph{inherent confusion} amongst the labels for the instance $x$.

Given an $(x_n, y_n) \sim \Pr$,
the empirical risk~\eqref{eqn:empirical-risk-one-hot}
approximates 
the distribution
$\pStar( x_n )$
%which typically is supported on multiple labels,
with the one-hot $e_{y_n}$,
which is only supported on one label.
While this is an unbiased estimate,
it is a significant reduction in granularity. %of information.
By contrast,
consider the following \emph{Bayes-distilled risk} on a sample $S \sim \Pr^N$:
\begin{equation}
    \label{eqn:bayes-distillation}
    \RDistBayes( f; S ) \defEq \frac{1}{N} \sum_{n = 1}^N \pStar( x_n )^{\tup} \ell( f( x_n ) ).
\end{equation}
This is a distillation objective (cf.~\eqref{eqn:distillation-risk}) using a \emph{Bayes teacher},
who provides the student with the true class-probabilities.
Rather than fitting to a single label realisation $y_n \sim \pStar( x_n )$,
a student minimising~\eqref{eqn:bayes-distillation} considers all \emph{alternate} label realisations,
weighted by their likelihood.%
\footnote{While the student could trivially memorise the \emph{training} class-probabilities,
this would not generalise to \emph{test} samples.}
Observe that when $\ell$ is the cross-entropy,~\eqref{eqn:bayes-distillation}
is simply the KL divergence between the Bayes class-probabilities and our predictions.

Both the standard 
empirical risk
$\REmp( f; S )$ in~\eqref{eqn:empirical-risk-one-hot}
and Bayes-distilled risk $\RDistBayes( f; S )$ in~\eqref{eqn:bayes-distillation} 
are unbiased estimates of the population risk $R( f )$.
But intuitively, we expect that a student minimising~\eqref{eqn:bayes-distillation}
ought to generalise better from a finite sample.
We can make this intuition precise by establishing that the Bayes-distilled risk has \emph{lower variance},
considering fresh draws of the training sample.

%
\begin{lemma}
\label{lemm:lower-variance}
For any fixed predictor $f \colon \XCal \to \Real^{L}$,
$$ \mathbb{V}_{S \sim \Pr^{N}}\left[ \RDistBayes( f; S ) \right] \leq \mathbb{V}_{S \sim \Pr^{N}}\left[ \REmp( f; S ) \right], $$
where $\mathbb{V}$ denotes variance,
and equality holds iff 
$\forall x \in \XCal$,
the loss values
$\ell( f( x ) )$ are constant on the support of $\pStar( x )$.
\end{lemma}

%
\begin{proof}[Proof of Lemma~\ref{lemm:lower-variance}]
By definition,
\begin{align*}
    \mathrm{LHS} &= \frac{1}{N} \cdot \mathbb{V}\left[ \pStar( \X )^{\tup} \ell( f( \X ) ) \right] \\
    &= \frac{1}{N} \cdot \mathbb{V}\left[ \E{\Y \mid \X}{ \ell( \Y, f( \X ) ) } \right] \\
    &= \frac{1}{N} \cdot \ES{\X}{ \left[ \E{\Y \mid \X}{ \ell( \Y, f( \X ) ) } \right]^2 } -
    \frac{1}{N} \cdot \left[ \ES{\X}{\E{\Y \mid \X}{ \ell( \Y, f( \X ) ) }} \right]^2.
\end{align*}
% Similarly,
\begin{align*}
    \mathrm{RHS} &= \frac{1}{N} \cdot \mathbb{V}\left[ \ell( \Y, f( \X ) ) \right] \\
    &= \frac{1}{N} \cdot \ES{\X}{\E{\Y \mid \X}{ \ell( \Y, f( \X ) )^2 }} - \frac{1}{N} \cdot \left[ \ES{\X}{\E{\Y \mid \X}{ \ell( \Y, f( \X ) ) }} \right]^2.
\end{align*}
In both cases, the second term simply equals $R( f )^2$
since both estimates are unbiased.
For fixed $x \in \XCal$, 
the result follows by Jensen's inequality applied to the random variable 
$\Z \defEq \ell( \Y, f( x ) )$.
Equality occurs iff $\Z$ is constant,
which requires the loss to be constant on the support of $\pStar( x )$.
\end{proof}

The condition when the Bayes-distilled and empirical risks have the same variance is intuitive:
the two risks trivially agree
when $f$ is non-discriminative (attaining equal loss on all labels),
or when a label is inherently deterministic (the class-probability is concentrated on one label).
For discriminative predictors and non-deterministic labels,
however,
the Bayes-distilled risk can have significantly lower variance.

The reward of reducing variance is better generalisation:
a student minimising~\eqref{eqn:bayes-distillation},
will better minimise the population risk,
compared to using one-hot labels.
In fact, we may quantify how the \emph{empirical} variance of the Bayes-distilled loss values
influences generalisation as follows.

%
\begin{proposition}
\label{prop:svp}
Pick any bounded loss $\ell$.
Fix a hypothesis class $\FCal$ of predictors 
%$f \colon \XCal \to [ 0, 1 ]$
$f \colon \XCal \to \Real^L$,
with induced class $\HCal^* \subset [ 0, 1 ]^{\XCal}$ 
of functions $h( x ) \defEq \pStar( x )^{\tup} \ell( f( x ) )$.
Suppose $\HCal^*$
has uniform covering number 
%$\mathscr{N}_{\infty}( \epsilon, \HCal^*, n )$.
$\mathscr{N}_{\infty}$.
Then,
for any $\delta \in (0, 1)$,
with probability at least $1 - \delta$ over $S \sim \Pr^N$,
$$ R( f ) \leq \RDistBayes( f; S ) + \mathscr{O}\left( \sqrt{ \mathbb{V}^*_N( f ) \cdot \frac{\log \frac{\mathscr{M}^*_N}{\delta}}{N}} + \frac{\log \frac{\mathscr{M}^*_N}{\delta}}{N} \right), $$
where $\mathscr{M}^*_N \defEq \mathscr{N}_{\infty}( \frac{1}{N}, \HCal^*, 2 N )$
and $\mathbb{V}^*_N( f )$ is the empirical variance of the loss values $\{ \pStar( x_n )^{\tup} \ell( f( x_n ) ) \}_{n = 1}^N$.
\end{proposition}

%
\begin{proof}[Proof of Proposition~\ref{prop:svp}]
This a simple consequence of~\citet[Theorem 6]{Maurer:2009},
which is a uniform convergence version of Bennet's inequality~\citep{Bennett:1962}.
% See also~\citet[Theorem 4]{Audibert:2009}.
\end{proof}

% {\color{red}\LARGE Address the offline discussion....}
The above may be contrast to the
bound achievable for the standard empirical risk using one-hot labels:
by~\citet[Theorem 6]{Maurer:2009},
$$ R( f ) \leq \REmp( f; S ) + \mathscr{O}\left( \sqrt{ \mathbb{V}_N( f ) \cdot \frac{\log \frac{\mathscr{M}_N}{\delta}}{N}} + \frac{\log \frac{\mathscr{M}_N}{\delta}}{N} \right), $$
where here we consider a function class $\HCal$ comprising functions $h( x, y ) = e_{y}^{\tup} \ell( f( x ) )$,
with uniform covering number $\mathscr{M}_N$.
Combining the above with Lemma~\ref{lemm:lower-variance}, we see that the Bayes-distilled empirical risk results in a lower variance penalty.%
%{\color{red}\footnote{Since $\HCal^*$ comprises the convex hull of $\HCal$, the uniform covering number $\mathscr{M}^*_N = \mathscr{M}_N$.} \Large LET'S VERIFY THIS FOOTNOTE.}
%{\footnote{Since $\HCal^*$ comprises the convex hull of $\HCal$, the uniform covering number $\mathscr{M}^*_N = \mathscr{M}_N$.}}

%
To summarise the statistical perspective
espoused above,
a student should ideally have access to the underlying class-probabilities $\pStar( x )$,
rather than a single realisation $y \sim \pStar( x )$.
% When $\pStar( x )$ has significant mass on more than one labels,
% our classification problem has \emph{inherent label noise}.
% {Compared to the empirical risk,~\eqref{eqn:bayes-distillation} offers more information: %can be understood as a specific form of data augmentation:
% rather than observing a single ``true'' label for a given $x$,
% we observe infinitely many ``noisy'' labels,
% %from which we can reliably estimate the true $\pStar( x )$.
% which in aggregate help better discriminate amongst instances.
% }
%Our analysis in~\S\ref{sec:bayes-distillation} provides 
As a final comment, the above provides
a statistical perspective on the value of ``dark knowledge'':
the teacher's ``wrong'' logits $y' \neq y$ for an example $(x, y)$
provide approximate information about the Bayes class-probabilities.
This results in a lower-variance student objective, %than the standard empirical risk,
aiding generalisation.

%
%\subsection{Distillation through a class-probability lens}
\subsection{Distilling from an imperfect teacher}
\label{sec:bias-variance}

\input{bias_variance}


%
\subsection{Discussion and implications}

Our statistical perspective gives a simple yet powerful means of understanding distillation.
Our formal results follow readily from this perspective,
but their implications are subtle, and merit further discussion.

%
% The above raises several points that are worth discussing.
$\triangleright$ \emph{Why accuracy is not enough}.
Our bias-variance result %in~\S\ref{sec:bias-variance} 
establishes that if the teacher provides good class-probabilities,
in the sense of approximating $\pStar$ in a mean-square sense,
then the resulting student should generalise well.
In deep networks,
this does
\emph{not} imply providing the teacher having higher accuracy;
such models
may be accurate while being overly confident%
%meaning their probabilities are poorly calibrated
~\citep{Guo:2017,Rothfuss:2019}.
Our result thus potentially illuminates why more accurate teachers may lead to poorer students,
as has been noted empirically~\citep{Muller:2019};
see also~\S\ref{sec:bias-variance-cifar100}. 
%and~\S\ref{sec:distorted_bayes_distillation}.

In practice,
the precise bound derived above is expected to be loose.
However, its qualitative trend may be observed in practice.
Figure~\ref{fig:cifar100-distillation} (see also~\S\ref{sec:bias-variance-cifar100}) illustrates 
how increasing the depth of a ResNet model may increase accuracy, but degrade probabilistic calibration.
This is seen to directly relate to the quality of a student distilled from these models.

Temperature scaling~\citep{Hinton:2015}, a very common and empirically successful trick in distillation, 
can also be analysed through this perspective. 
Usually, teachers are highly complex and optimised to maximise accuracy; hence, they often become overly confident. 
Increasing the temperature can help the student-target 
be closer to the true distribution, 
and not just convey the most accurate label.

%
$\triangleright$ \emph{Teacher variance and model capacity}.
%One subtle difference to the previous section is that
Proposition~\ref{prop:bias-variance} allows for $\pTeach$ to be random (e.g., owing to the teacher being learned from some independent sample $S^{\mathrm{t}} \sim \Pr^{N^{\mathrm{t}}}$).
Consequently, 
the variance terms not only reflect how diffused the teacher's predictions are,
{but}
also how much these predictions \emph{vary} over fresh draws of the \emph{teacher} sample.
\emph{High-capacity} teachers may yield vastly different predictions when trained on fresh samples.
This variability incurs a penalty in the third term in Proposition~\ref{prop:bias-variance}.
At the same time, such teachers can better estimate the Bayes $\pStar( x )$,
which incurs a lower bias.
% As with standard learning, 
The delicate tradeoff between these concerns translates into (student) generalisation.

%
We may understand
the %popular
\emph{label smoothing} trick~\citep{Szegedy:2016}
in light of the above.
This corresponds to 
mixing the student labels with uniform predictions, yielding
$\pTeach( x ) = (1 - \alpha) \cdot e_{y} + \frac{\alpha}{L} \cdot \mathbf{1}$
for $\alpha \in [ 0, 1 ]$.
From the perspective of modelling $\pStar$, 
choosing $\alpha > 0 $ introduces a \emph{bias}.
{However},
$\pTeach( x )$ has lower \emph{variance} than the one-hot labels $e_y$'s,
owing to the $(1 - \alpha)$ scaling.
% and $\frac{\alpha}{L} \cdot \mathbf{1}$ is a constant.
Provided the bias is not too large, 
smoothing can thus aid generalisation.

We remark also that the first variance term in Proposition~\ref{prop:bias-variance} 
vanishes as $N \to \infty$.
This is intuitive: in the limit of infinite student samples,
the quality of the distilled objective is wholly determined by how well the teacher probabilities model the Bayes probabilities.
For small $N$, 
this term measures how diffused the losses are when weighted by the teacher probabilities (similar to Lemma~\ref{lemm:lower-variance}).

%
$\triangleright$ \emph{How much teacher bias is admissible?}
When $\pTeach \neq \pStar$,
Proposition~\ref{prop:bias-variance} 
reveals that a distilled student's generalisation gap depends on the bias and variance in $\pTeach$.
By contrast,
from a labelled sample, 
the student's generalisation gap depends on the complexity of its model class $\FCal$.
Distillation can be expected to help when the first gap is lower than the second.

Concretely, 
when trained from limited labelled samples, the student will find
$\min_{f \in \FCal} \hat{R}( f; S )$,
which incurs a high \emph{statistical} error.
Now
suppose we have a large amount of unlabelled data $N \to \infty$.
A distilled student can then reliably find the minimiser (following~\eqref{eqn:risk-as-divergence})
$$ \min_{f \in \FCal} \E{\X}{ D( \pTeach( \X ) \| f( \X )  ) }, $$
with essentially no statistical error,
but an \emph{approximation} error given by the teacher's bias.
In this setting, we thus need
\emph{the teacher's bias to be lower than the statistical error}.

%
$\triangleright$ \emph{On teacher versus student samples}
A qualifier to our results is that they assume a disjoint set of samples for the teacher and student.
For example, it may be that the teacher is trained on a pool of labelled samples,
while the student is trained on a larger pool of unlabelled samples.
The results thus do not directly hold for the settings of \emph{self-} or \emph{co-}distillation~\citep{Furlanello:2018,Anil:2018},
wherein the same sample is used for both models.
Combining our results with recent analyses
from the perspective of regularisation~\citep{Mobahi:2020} and 
data-dependent function classes~\citep{Foster:2019} would be of interest in future work.


% Formally, 
% the variance term in Proposition~\ref{prop:bias-variance} is negligible in this setting.

% Thus, 
% % The quality of risk approximation 
% ~\eqref{eqn:bias-variance-generalisation}
% will be dominated by the teacher's $\pTeach$.
% This bias must thus be \emph{smaller}
% than the penalty obtained from \emph{standard} training on one-hot labelled samples.

% This minimiser has potentially two sources of error:
% that from the approximate nature of $\pTeach$,
% and
% that from the inability of $\FCal^{\mathrm{s}}$ to model $\pTeach$.

% Nonetheless, this solution may be superior to that 
% the student can obtain from a small number of labelled samples alone, 
% i.e.,
% $\min_{f \in \FCal} \hat{R}( f; S )$.
%$$ \min_{f \in \FCal^{\mathrm{s}}} \E{\X}{ D( \pStar( \X ) \| f( \X )  ) }. $$

% %
% \subsection{Distillation and label smoothing}

% Given a training sample $\{ ( x_n, y_n ) \}_{n = 1}^N \sim \Pr^N$,
% the standard empirical risk is
% \begin{align*}
%     \REmp( f; S ) &\defEq \frac{1}{N} \sum_{n \in [N]} \ell( y_n, f( x_n ) ) \\
%     &= \frac{1}{N} \sum_{n \in [N]} \sum_{y \in [L]} \indicator{ y_n = y } \cdot \ell( y, f( x_n ) ).
% \end{align*}
% Now suppose we have class-probability estimates $\hat{p}( x ) \in \Delta_L$ for each training sample,
% as produced, e.g., from some teacher model.
% Then, we may construct the distillation objective
% \begin{align*}
% \RDist( f; S ) &= \frac{1}{N} \sum_{n \in [N]} \sum_{y \in [L]} [ \hat{p}( x_n ) ]_y \cdot \ell( y, f( x_n ) ) \\
% &= \frac{1}{N} \sum_{n \in [N]} \E{\Y \sim \hat{p}( x_n )}{ \ell( \Y, f( x_n ) ) } \\
% &={\color{red}\frac{1}{N} \sum_{n \in [N]}\hat{p}( x_n )^\tup{ \ell(f( x_n ) ) }}
% \end{align*}
% The empirical risk is thus the special case where each $\hat{p}( x )$ is a delta function.
% {\color{blue}Compared to the empirical risk, distillation can be understood as performing a kind of data augmentation:
% rather than observe a single label for a given $x_i$,
% we effectively observe infinitely many labels,
% from which we can estimate the true class-conditional probability.} \ankit{Is this really data augmentation? Perhaps, it's more like receiving a large number of noisy samples -- which is much better than receiving a single clean sample?}

% {\bf\color{red} TODO: convert to generalisation bound.}

% To understand this result intuitively,
% observe that we can rewrite the population risk as
% $$ R( f ) = \E{\X}{ \pStar( \X )^{\tup} \ell( f( \X ) ) }, $$
% {\color{blue}where in an abuse of notation $\ell( f ) = [ \ell( y, f(x) ) ]_{y \in \YCal} \in \Real^L$ is the vector of losses for all possible labels,
% and $\pStar( x ) \defEq \Pr( \Y \mid \X = x ) \in \Delta_L$ is the vector of class-probabilities for all possible labels.} \ankit{Already defined in the background section.}

% Ideally, we would have access to instances $\X \sim \Pr_{\X}$,
% and their corresponding class-probability vectors $\pStar( \X )$.
% However, in practice we only have access to instances $\X \sim \Pr_{\X}$ and a single label $\Y \sim \pStar( \X )$.
% This corresponds to using a one-hot empirical estimate $\mathbf{e}_{\Y}$ in place of $\pStar( \X )$.
% One consequence of distillation, however, is that we can better approximate $\pStar( \X )$ by {\color{red}$\hat{p}(\X)$}, thereby reducing the variance of our estimate of the population risk {\color{red}(as long as $\hat{p}(\X)$ is close to $\pStar( \X )$)}.

% It is elementary to see that
% both risks are unbiased,
% i.e.,
% $\E{S \sim \Pr^{N}}{ \REmp( f; S ) } = \E{S \sim \Pr^{N}}{ \RDistBayes( f; S ) } = R( f )$.
% Consequently,
% it suffices to establish
% that
% $$ \E{S \sim \Pr^{N}}{ \RDistBayes( f; S )^2 } \leq \E{S \sim \Pr^{N}}{ \REmp( f; S )^2 }. $$
% For brevity, let $z_*( x ) \defEq \pStar( x )^{\tup} \ell( f( x ) )$.
% Evidently,
% \begin{align*}
% \mathrm{LHS} &= \frac{1}{N^2} \cdot \E{}{ \sum_{n} z_*( x_n )^2 + \sum_{n \neq m} z_*( x_n ) \cdot z_*( x_m ) } \\
% &= \frac{1}{N} \cdot \E{}{ (z_*( \X ))^2 } + \frac{N \cdot (N - 1)}{N^2} \cdot \E{}{ z_*( \X ) }^2.
% \end{align*}
% Similarly,
% for $z( x, y ) \defEq e_y^{\tup} \ell( f( x ) )$,
% \begin{align*}
% \mathrm{RHS} &= \frac{1}{N} \cdot \E{}{ (z( \X, \Y ))^2 } + \frac{N \cdot (N - 1)}{N^2} \cdot \E{}{ z( \X, \Y ) }^2.
% \end{align*}

% Note that 
% \begin{align}
% \label{eq:var-emp}
% \mathbb{V}( \REmp( f; S )) &= \frac{1}{N}\cdot \bigg( \E{(\X, \Y) \sim \Pr}{ \left( \ell( \Y, f( \X ) ) \right)^2 } - \nonumber \\
% &\qquad \qquad \E{(\X, \Y) \sim \Pr}{ \ell( \Y, f( \X ) ) }^2\bigg),
% \end{align}
% where, for a random sample of an instance and a label,
% \begin{align*}
%     \E{(\X, \Y) \sim \Pr}{ \ell( \Y, f( \X ) ) } &= R( f ) \\
%     \E{(\X, \Y) \sim \Pr}{ \left( \ell( \Y, f( \X ) ) \right)^2 } &= \E{\X \sim \Pr_{\X}}{ \sum_{y \in [L]} \pStar_y( \X ) \cdot \ell( y, f( \X ) )^2 }.
% \end{align*}
% On the other hand, for the Bayes-distillation objective, we have 
% \begin{align}
% \label{eq:var-dist}
% \mathbb{V}( \RDist( f; S )) &= \frac{1}{N}\cdot \bigg( \E{\X \sim \Pr_{\X}}{ \left( \hat{p}(\X)^T\ell(f( \X ) ) \right)^2 } - \nonumber \\
% &\qquad \quad\E{\X \sim \Pr_{\X}}{\hat{p}(\X)^T\ell(f( \X ) )  }^2\bigg).
% \end{align}
% Let's assume that we have access to the true class probability for the distillation, i.e., $\hat{p}(\X) = \pStar(\X)$. Note that
% %if we only draw a random instance, but employ its true class-probability distribution,
% \begin{align*}
%     \E{\X \sim \Pr_{\X}}{ \pStar( \X )^{\tup} \ell( f( \X ) ) } &= R( f ) \\
%     \E{\X \sim \Pr_{\X}}{ \left( \pStar( \X )^{\tup} \ell( f( \X ) ) \right)^2 } &= \E{\X \sim \Pr_{\X}}{ \sum_{y \in [L]} (\pStar_y( \X ))^{2} \cdot \ell( y, f( \X ) )^2 }.
% \end{align*}
% In this case, $\mathbb{V}( \RDist( f; S ))$ is strictly smaller than $\mathbb{V}( \REmp( f; S ))$ since $(\pStar_y( \X ))^{2} \leq \pStar_y( \X )$.
% %Observe that in the latter case, we thus have a strictly smaller variance since $(\pStar_y( \X ))^{2} \leq \pStar_y( \X )$.
% {\color{blue}The variance reduction is maximal when the class-probabilities are close to uniform, i.e., the underlying problem has higher noise.}

% To make this precise,
% consider a student which has access to a training sample $S = \{ ( x_n, y_n ) \}_{n = 1}^{N}$.
% The student's baseline performance is its predictor learned by minimising the empirical risk $\REmp( f; S )$.
% But now suppose the student has access to an \emph{oracle teacher},
% who provides them with the sample $S' = \{ ( x_n, \pStar( x_n ) ) \}_{n = 1}^N$,
% where each $x_n$ is annotated with the \emph{true class-probabilities} for each possible label.
% Can the student learn a better predictor from $S'$?


==> Why distillation helps ICML 2020/background.tex <==
We review
multiclass classification, 
%multiclass 
retrieval, 
\&
distillation.

%
\subsection{Multiclass classification}

In multiclass classification,
we are given
a training sample $S \defEq \{ ( x_n, y_n ) \}_{n = 1}^N \sim \Pr^N$,
for unknown distribution $\Pr$ over instances $\XCal$ and labels $\YCal = [ L ] \defEq \{ 1, 2, \ldots, L \}$.
Our goal is to learn a predictor $f \colon \XCal \to \Real^L$ so as to minimise the \emph{risk} of $f$, i.e., its expected {loss} for a random instance and label:
\begin{equation}
    \label{eqn:risk}
    R( f ) \defEq \E{(\X, \Y) \sim \Pr}{ \ell( \Y, f( \X ) ) }.
\end{equation}
Here, $\ell \colon [ L ] \times \Real^L \to \Real_+$ is a loss function, 
where
for label $y \in [ L ]$ and prediction vector $f(x) \in \Real^L$,
$\ell( y, f(x) )$ is the loss incurred for predicting $f(x)$ when the true label is $y$.
A canonical example is
the softmax cross-entropy loss,
\begin{equation}
    \label{eqn:softmax-xent}
    \ell( y, f( x ) ) = -f_y( x ) + \log \left[ \sum_{y' \in [ L ]} e^{f_{y'}( x )} \right].
\end{equation}
% Given the training sample $S$, we replace $R( f )$ with
We may approximate {the risk} $R( f )$ %on $S$ via 
via
the \emph{empirical risk} %$\REmp( f; S )$
\begin{equation}
    \label{eqn:empirical-risk-one-hot}
    %\resizebox{0.9\linewidth}{!}{$\displaystyle
    \REmp( f; S ) \defEq \frac{1}{N} \sum_{n \in [N]} \ell( y_n, f( x_n ) ) %\\
    = \frac{1}{N} \sum_{n \in [N]} e_{y_n}^{\tup} \ell( f( x_n ) ),
    %$}
\end{equation}
where 
${e}_y \in \{ 0, 1 \}^L$ denotes the one-hot encoding of $y \in [ L ]$ and %, with an abuse of notation,
{$\ell( f(x) ) \defEq \big(\ell(1, f(x)),\ldots, \ell(L, f(x))\big)\in \Real_+^L$} denotes the vector of losses
for each possible label.

In a multiclass \emph{retrieval} setting,
our goal is to ensure that the top-ranked labels in $f( x ) \in \Real^L$ include the true label~\citep{Lapin:2018}. %~\citep{Lapin:2018,Reddi:2019,Guo:2019}.
Formally, we seek to minimise
the
\emph{top-$k$ loss}
\begin{equation}
    \label{eqn:top-k-risk}
    %R_{\mathrm{ret}}( f ) 
    %\defEq \E{( \X, \Y ) \sim \Pr}{ \ell_{\mathrm{ret}(r)}( \Y, f( \X ) ) },
    \ell_{\mathrm{ret}(k)}( y, f( x ) ) \defEq \indicator{y \notin \mathrm{top}_k( f( x ) )},
\end{equation}
%where $\ell_{\mathrm{ret}(r)}( i, f ) \defEq \indicator{i \notin \mathrm{top}_r( f )}$, and 
where $\mathrm{top}_k( f )$ denotes the 
%indices of the $k$ labels with the highest scores under $f$.
top-$k$ highest scoring labels.
When $k = 1$, this loss reduces to the standard 0-1 error.
%{misclassification or 0-1 error}.

%
\subsection{Knowledge distillation}
\label{sec:background-distillation}

Distillation involves using a ``teacher'' model to improve the performance of a  ``student'' model~\citep{Bucilua:2006,Hinton:2015}.
In the simplest form, one 
trains the teacher model and obtains
\emph{class-probability estimator} $\pTeach \colon \XCal \to \Delta_{\YCal}$,
where $\Delta$ denotes the simplex.
%Given an instance $x \in \XCal$, 
Each
$\pTeach_y( x )$ estimates how likely $x$ is to be classified as $y$.
% These estimates are then fed into the student
% in place of the raw labels:
% we replace the empirical risk~\eqref{eqn:empirical-risk-one-hot} with the
In place of the empirical risk~\eqref{eqn:empirical-risk-one-hot},
the student now minimises the
\emph{distilled risk}
\begin{equation}
    \label{eqn:distillation-risk}
    \RDist( f; S ) = \frac{1}{N} \sum_{n \in [N]} \pTeach( x_n )^\tup \ell(f( x_n ) ),
\end{equation}
so that the one-hot encoding of labels is replaced with the teacher's distribution over labels.
% When $\ell$ is the softmax cross-entropy,
% this is equivalent to minimising the KL divergence between the 
% teacher's distribution
% and the
% student's predictions.
% uses the teacher to produce an estimated label distribution $\mathbf{p}^{\mathrm{teach}}_y \in \Delta_{L}$,
% which is then fed as input into the student.
% This can be seen as a data-dependent form of label smoothing:
% the teacher model instructs the student as to potential alternatives to the observed label.
Distillation may be used 
when the student has access to a large pool of unlabelled samples;
in this case, distillation is a means of semi-supervised learning~\citep{Radosavovic:2018}.

While originally conceived 
in settings 
where the student has lower capacity than the teacher~\citep{Bucilua:2006,Hinton:2015},
distillation has proven useful when both models have the same capacity~\citep{Breiman:1996,Furlanello:2018,Xie:2019}.
% ARXIV
More precisely, distillation involves training a teacher on $N_t$ labelled samples $S^{\mathrm{t}} \sim \Pr^{N^{\mathrm{t}}}$,
using a function class $\FCal^{\mathrm{t}}$.
Classic distillation assumes that $N^{\mathrm{t}} \gg N$, and that the capacity of $\FCal^{\mathrm{t}}$ is greater than that of $\FCal$.
``Born-again'' distillation assumes that $S^{\mathrm{t}} = S$, and $\FCal^{\mathrm{t}} = \FCal$,
i.e.,
one iteratively trains versions of the same model, using past predictions to improve performance.

%
\subsection{Existing explanations for distillation}

While 
it is well-accepted that
distillation is empirically useful,
there is less consensus
as to \emph{why} this is the case.
\citet{Hinton:2015} attributed the success of distillation (at least in part) to the encoding of ``dark knowledge'' 
in the probabilities the teacher
assigns to the ``wrong'' labels $y' \neq y$ for example $(x, y)$.
% which states that the teacher transfers knowledge about the  for an instance to the student.
This richer information plausibly aids the student,
providing for example a weighting on the samples~\citep{Furlanello:2018,Tang:2020}.
Further, 
when $\ell$ is
the softmax cross-entropy,
the gradient of the distillation objective with respect to the student logits is 
the difference in the probability estimates for the two, 
implying a form of logit matching in high-temperature regimes~\citep{Hinton:2015}.

%There have been more formal analyses of distillation.
\citet{Lopez-Paz:2016} related distillation to learning from privileged information under a noise-free setting.
~\citet{Phuong:2019} analysed the dynamics of student learning, 
assuming a deep linear model for binary classification.
~\citet{Foster:2019} provided a generalisation bound for the student, under the assumption that it learns a model close to the teacher.
This does not, however, explicate what constitutes an ``ideal'' teacher,
nor quantify how an approximation to this ideal teacher will affect the student generalisation. \citet{Gotmare:2019} studied the effect of distillation on discrimination versus feature extraction layers of the student network.
\citep{Dong:2019} argued that distillation has a similar effect to early stopping, and studied its ability to denoise labels.
Our focus, by contrast, is in settings where there is no exogenous label noise, and in studying the statistical rather than optimisation effects of distillation.
\citep{Mobahi:2020} analysed the special setting of \emph{self-distillation} -- wherein the student and teacher employ the same model class -- and showed that for kernelised models, this is equivalent to increasing the regularisation strength.

% ARXIV
% In sum,
% while each of these are illuminating,
% a complete picture of why and when distillation helps
% remains elusive.

% Recently,
% \citet{Muller:2019} explored the relationship between distillation and label smoothing~\citep{Szegedy:2016}.
% In particular, they established that distillation can offer superior performance to oblivious smoothing of the student model.
% Further, they established that smoothing on the teacher model can impair performance.

% This serves as an unbiased estimate of the population risk $R( f )$.
% Generalisation bounds relate the empirical and population risks, and typically are of the form~\citep{Boucheron:2005}
% $$ \Pr_{S}\left[ R( f ) \leq \REmp( f; S ) + \mathrm{comp}( \mathscr{F}, N, \delta ) \right] \geq 1 - \delta $$
% where $\mathrm{comp}( \mathscr{F}, N, \delta )$ is a measure of complexity of the underlying function class $\mathscr{F} \subset \Real^{\XCal}$,
% sample size $N$, and error probability $\delta \in ( 0, 1 )$.
% A classical complexity bound is $\sqrt{ \frac{\mathrm{VC}( \mathscr{F} )}{N} \cdot \log \frac{1}{\delta} }$,
% where $\mathrm{VC}( \cdot )$ denotes the VC-dimension of a function class~\citep{Vapnik:1995}. \ankit{Maybe state the Rademacher version.}

% %
% \subsection{Multiclass retrieval}

% In multiclass retrieval,
% our goal is to find an $f$ that minimises the \emph{retrieval risk}, 


% In practice, directly minimising $L_{\mathrm{ret}(r)}( f )$ is computationally prohibitive
% owing to the non-differentiability of the loss $\ell_{\mathrm{ret}( r )}$.
% This can be alleviated by minimising a suitable \emph{surrogate} loss $\ell \colon [ L ] \times \Real^L \to \Real_+$.
% Examples of $\ell$ include the softmax cross-entropy 
% $\ell( y, f( x ) ) = -f_y( x ) + \log \sum_{y'} e^{f_{y'}( x )}$,
% and %the family of 
% \emph{binary ordered weighted losses} (\emph{BOWLs})~\citep{Reddi:2019}
% \begin{equation}
%     \label{eqn:bowl}
%     \ell( y, f( x ) ) = \phi( f_y( x ) ) + \mathrm{avg}_{\mathrm{top}( k )}\left( \{ \phi( -f_{y'}( x ) ) \}_{y' \neq y} \right),
% \end{equation}
% where 
% $\phi \colon \Real \to \Real_+$ is a margin loss,
% $k$ is an integer,
% and $\mathrm{avg}_{\mathrm{top}( k )}$ denotes the average of the top-$k$ largest elements of a vector.
% When $k = 1$,
% we obtain the Crammer-Singer loss~\citep{Crammer:2002},
% \begin{equation}
%     \label{eqn:cs-loss}
%     \ell( y, f( x ) ) = \phi( f_y( x ) ) + \max_{y' \neq y} \phi( -f_{y'}( x ) ).
% \end{equation}
% This provides a tight bound on $L_{\mathrm{top}(1)}( f )$.
% When $k = L - 1$,
% we obtain the averaged loss~\citep{Zhang:2004b},
% \begin{equation}
%     \label{eqn:ova}
%     \ell( y, f( x ) ) = \phi( f_y( x ) ) + \frac{1}{L - 1} \sum_{j \neq y} \phi( -f_j( x ) ).
% \end{equation}
% Given a training sample $S \defEq \{ ( x_n, y_n ) \}_{n \in [N]} \sim \Pr^N$
% and loss $\ell$,
% one may seek to minimise the empirical risk
% \begin{equation}
%     \label{eqn:empirical-risk}
%     \REmp( f; S ) \defEq \frac{1}{N} \sum_{i \in [N]} \ell( y_i, f( x_i ) ).
% \end{equation}

% %
% \subsection{Label smoothing}

% Observe that we may write the loss for a given label as
% $\ell( y, f(x) ) = \mathbf{e}_y^{\tup} \ell( f(x) )$, where 
% $\mathbf{e}_y \in \{ 0, 1 \}^L$ is the one-hot encoding of $y$, and {\color{red}$\ell( f(x) ) = \big(\ell(1, f(x)),\ldots, \ell(L, f(x))\big)\in \Real_+^L$} is the vector of losses. In label smoothing~\citep{Szegedy:2016}, one replaces this encoding with a generic distribution $\mathbf{p}_y \in \Delta_L$, yielding a \emph{smoothed loss} $\ell_{\mathrm{sm}}( y, f ) = \mathbf{p}_y^{\tup} \ell( f(X) )$.

% From the previous section, 
% for a training sample $(x, y)$,
% we should ideally pick $\mathbf{p}_y$ to be {\color{red}$\mathbf{p}^*( x ) \defEq \Pr[Y| X = x]$.} \ankit{Maybe denote this by $\mathbf{p}_y^{*,x}$ OR simply $\mathbf{\bar{p}}_y^{x}$? In any case, $y$ in the subscript is necessary to be consistent. Reading the rest of the sections, I feel like we should just drop the subscript here, because we use $y$ as the summation index later one :)}
% However, given this quantity is unknown, we must settle for surrogates.
% Options include:
% \begin{itemize}[itemsep=0pt,topsep=0pt]
%     \item \emph{Oblivious smoothing}. Suppose that $\mathbf{p}_y = (1 - \alpha) \cdot \mathbf{e}_y + \frac{\alpha}{L} \cdot \mathbf{1}$ for some $\alpha \in (0, 1)$.
% This corresponds to mixing the true label with a uniform distribution over all the classes.

%     \item \emph{Mixup smoothing}. One form of data-dependent smoothing, 
% which we call \emph{mixup smoothing}~\citet{Zhang:2018},
% involves taking pairs of instances \emph{and} labels, and linearly interpolating between them.
% In label space, this corresponds to using $\mathbf{p}_y = (1 - \alpha) \cdot \mathbf{e}_y + \alpha \cdot \mathbf{e}_{y'}$ for some other $(x', y')$ in the training sample. \ankit{Mixup also interpolates the instance?}
% \end{itemize}

% %
% \subsection{Extreme classification}
% \label{sec:background-retrieval}

% The \XLC{} setting refers to multiclass problems where the number of possible labels $L$ is large (e.g., the order of billions)~\citep{Prabhu:2018,Jain:2019,Reddi:2019,Guo:2019}.
% This poses a challenge for training standard models
% since even computing $\ell( y, f( x ) )$ for a \emph{single} pair $(x, y)$ can be prohibitive.
% To see this, note e.g.\ that in the softmax cross-entropy~\eqref{eqn:softmax-xent},
% computing the loss requires the score of \emph{all} possible labels.

% This motivates \emph{negative mining} techniques~\citep{Sung:1996,Dalal:2005,Felzenszwalb:2010},
% which select a suitable subsample of the labels.
% For example, \emph{sampled softmax} techniques seek
% to construct a model of label scores which can be efficiently sampled from~\citep{Bengio:2008,Jean:2015,Blanc:2018,Rawat:2019}.
% Similarly,
% for losses other than the softmax cross-entropy,
% \emph{stochastic negative mining} proceeds by 
% focussing on only the ``hardest'' few labels from a randomly drawn subset~\citep{Reddi:2019}.


% One such choice of $\ell$ is the family of
% \emph{binary ordered weighted losses} (\emph{BOWLs})~\citep{Usunier:2009,Reddi:2019}
% \begin{equation}
%     \label{eqn:bowl}
%     \ell( y, f( x ) ) = \phi( f_y( x ) ) + \mathrm{avg}_{\mathrm{top}( k )}\left( \{ \phi( -f_{y'}( x ) ) \}_{y' \neq y} \right),
% \end{equation}
% where 
% $\phi \colon \Real \to \Real_+$ is a margin loss,
% $k$ is an integer,
% and $\mathrm{avg}_{\mathrm{top}( k )}$ denotes the average of the top-$k$ largest elements of a vector.
% When $k = 1$,
% we obtain the Crammer-Singer loss~\citep{Crammer:2002},
% \begin{equation}
%     \label{eqn:cs-loss}
%     \ell( y, f( x ) ) = \phi( f_y( x ) ) + \max_{y' \neq y} \phi( -f_{y'}( x ) ).
% \end{equation}


==> Why distillation helps ICML 2020/bias_variance.tex <==
The previous section explicates how an idealised ``Bayes teacher''
can be beneficial to a student.
How does this translate to more realistic settings, where one obtains predictions from a teacher which itself is learned form data?

Our first observation is that
a teacher's predictor $\pTeach$ can typically be seen as an 
imperfect estimate of the true $\pStar$.
Indeed, if the teacher is trained with a loss that is \emph{proper}~\citep{Savage:1971,Schervish:1989,Buja:2005}, %Gneiting:2007,Reid:2010},
then
\begin{equation}
    \label{eqn:risk-as-divergence}
    R( f ) = \E{\X}{ D( \pStar( \X ) \| \pTeach( \X ) ) } + \mathrm{constant},
\end{equation}
where $D( \cdot \| \cdot )$ is a (loss-dependent) \emph{divergence} between the true and estimated class-probability functions.
For example, the softmax cross-entropy corresponds to $D( \cdot \| \cdot )$ being the KL divergence between the distributions.
The teacher's goal is thus fundamentally to ensure that their predictions align with the true class-probability function.

Of course,
a teacher learned from finite samples is unlikely to achieve zero divergence in~\eqref{eqn:risk-as-divergence}.
Indeed, even high-capacity teacher models may not be rich enough capture the true $\pStar$.
Further, even if the teacher can represent $\pStar$,
it may not be able to \emph{learn} this perfectly given a finite sample,
owing to both 
statistical (e.g., the risk of overfitting) and 
optimisation (e.g., non-convexity of the objective) issues.
We must thus treat $\pTeach$ as an \emph{imperfect} estimate of $\pStar$.
The natural question is:
will such an estimate still improve generalisation?

To answer this,
we establish a fundamental \emph{bias-variance} tradeoff when performing distillation.
Specifically, we show the difference between the distilled risk $\RDist( f; S )$ (cf.~\eqref{eqn:distillation-risk}) and population risks $R( f )$ (cf.~\eqref{eq:population_risk})
depends on how variable the loss under the teacher is,
and how well the teacher estimates $\pStar$ in a squared-error sense. Intuitively, the latter captures how well the teacher estimates $\pStar$ on average (bias),
and how variable the teacher's predictions are (variance).
%
\begin{proposition}
\label{prop:bias-variance}
Pick any bounded loss $\ell$.
Suppose we have a teacher model $\pTeach$ with corresponding distilled empirical risk in \eqref{eqn:distillation-risk}.
For constant $C > 0$
and any predictor $f \colon \XCal \to \Real^L$,
% \begin{align*}
% \E{}{ ( \RDist( f; S ) - R( f ) )^2 } &\leq \frac{1}{N} \cdot \mathbb{V}\left[  \pTeach( \X )^{\tup} \ell( f( \X ) ) \right] + \\
% &C \cdot \left( \E{}{ \| \pTeach( \X ) - \pStar( \X ) \|_2 } \right)^2.
% \end{align*}
% ARXIV
\begin{align}
\label{eq:bias-variance-1}
\E{}{ ( \RDist( f; S ) - R( f ) )^2 } &\leq \frac{1}{N} \cdot \mathbb{V}\left[  \pTeach( \X )^{\tup} \ell( f( \X ) ) \right] + C \cdot \left( \E{}{ \| \pTeach( \X ) - \pStar( \X ) \|_2 } \right)^2 \\
&\leq \frac{1}{N} \cdot \mathbb{V}\left[  \pTeach( \X )^{\tup} \ell( f( \X ) ) \right] + C \cdot \left( { \| \E{}{ \pTeach( \X ) } - \pStar( \X ) \|_2^2 } + \mathbb{V}\left[ \pTeach( \X ) \right] \right), \label{eq:bias-variance-2}
\end{align}
where $\mathbb{V}\left[ \cdot \right]$ denotes the sum of coordinate-wise variance.
\end{proposition}

%
\begin{proof}[Proof of Proposition~\ref{prop:bias-variance}]
Let $\Delta \defEq \RDist( f; S ) - R( f )$. 
Then,
\begin{align*}
    \E{}{ ( \RDist( f; S ) - R( f ) )^2 } &= \E{}{ \Delta^2 } = \mathbb{V}[ \Delta ] + \E{}{ \Delta }^2.
\end{align*}
Observe that
\begin{align*}
    \E{}{ \Delta } &= \E{\X}{ (\pTeach( \X ) - \pStar( \X ))^{\tup} \ell( f( \X ) ) } \\
    &\leq \E{\X}{ \| \pTeach( \X ) - \pStar( \X ) \|_2 \cdot \| \ell( f( \X ) ) \|_2 } \\
    &\leq \E{\X}{ \| \pTeach( \X ) - \pStar( \X ) \|_2 \cdot C \cdot \| \ell( f( \X ) ) \|_{\infty} } \\
    &\leq C \cdot \E{\X}{ \| \pTeach( \X ) - \pStar( \X ) \|_2 },
\end{align*}
where the second line is by the Cauchy-Schwartz inequality,
and the third line by the equivalence of norms.
Now, \eqref{eq:bias-variance-1} follows since $R( f )$ is a constant, implying
\begin{align*}
\mathbb{V}[ \Delta ] &= \mathbb{V}[ \RDist( f; S ) ] = \frac{1}{N} \cdot \mathbb{V}\left[  \pTeach( \X )^{\tup} \ell( f( \X ) ) \right].
\end{align*}
For \eqref{eq:bias-variance-2}, by Jensen's inequality,
and the definition of variance,
\begin{align*}
    \left( \E{\X}{ \| \pTeach( \X ) - \pStar( \X ) \|_2 } \right)^2 &\leq \E{\X}{ \| \pTeach( \X ) - \pStar( \X ) \|_2^2 } \\
    &= \| \E{}{ \pTeach( \X ) } - \pStar( \X ) \|_2^2 + \mathbb{V}\left[ \pTeach( \X ) \right].
\end{align*}
\end{proof}

Unpacking the above, the fidelity of the distilled risk's approximation to the true one depends on three factors:
how variable the expected loss is for a random instance; how well the teacher's $\pTeach$ approximates the true $\pStar$ on average; and how variable the teacher's predictions are.
% , in a squared-error sense.
Mirroring the previous section,
we may convert Proposition~\ref{prop:bias-variance}
into a generalisation bound for the student:
\begin{equation}
    \label{eqn:bias-variance-generalisation}
    %\resizebox{0.9\linewidth}{!}{$\displaystyle
    R( f ) \leq \RDist( f; S ) + \mathfrak{C}( \FCal, N ) + \mathscr{O}\left(\mathbb{E}{}{ \| \pTeach( \X ) - \pStar( \X ) \|_2}\right),
    %$}
\end{equation}
where 
$\mathfrak{C}$ is the penalty term from Proposition~\ref{prop:svp}.
As is intuitive, using an imperfect teacher invokes an additional penalty depending on how far the predictions are from the Bayes, in a squared-error sense. For completeness, a formal statement is provided in Proposition~\ref{prop:svp-phat} in Appendix~\ref{sec:appendix-theory}.


==> Why distillation helps ICML 2020/body.tex <==
% !TEX root=./double_distillation.tex

%
\begin{abstract}
\input{abstract}
\end{abstract}

%
\section{Introduction}
\input{intro}

%
\section{Background and notation}
\input{background}

%
%\section{Distillation as variance reduction}
\section{Distillation through a class-probability lens}
\label{sec:analysis}
\input{analysis}

%
%\section{Double distillation for multiclass retrieval}
%\section{Distillation meets \XLC{}}
\section{Distillation meets multiclass retrieval}
\label{sec:double_distillation}
\input{double_distillation}

%
\section{Experimental results}
\label{sec:experiments}
\input{experiments}

%
\section{Conclusion}
\input{conclusion}


==> Why distillation helps ICML 2020/conclusion.tex <==
We presented a statistical perspective on distillation,
building on a simple observation:
\emph{distilling the Bayes class-probabilities yields a more reliable estimate of the population risk}.
Viewing distillation in this light, we formalised a bias-variance tradeoff to quantify the effect of approximate teacher class-probability estimates on student generalisation,
and also studied a novel application of distillation to \XLR{}.
Towards developing a comprehensive understanding of distillation,
studying the optimisation aspects of this viewpoint,
and the setting of overparametrised teacher models~\citep{Zhang:2018} would be of interest.

% In this paper,
% we present a statistical perspective on distillation
% which sheds light on why it aids performance,
% and provides a novel application to \XLR{}.
% Our analysis
% centers on a simple observation:
% \emph{the teacher's label probabilities can be seen as estimates of the true} (Bayes-optimal) \emph{class-probability function}.
% Motivated by this,
% we characterise how 
% access to
% such class-probability estimates can 
% significantly improve generalisation
% compared to learning from raw labels alone.
% We further propose a \emph{double-distillation} objective for selecting informative negative labels in \XLR{} problems.


==> Why distillation helps ICML 2020/double_distillation.tex <==
Our statistical view has thus far given insight into the potential value of distillation.
We now 
show a distinct practical benefit of this view, 
by leveraging it for a novel application of distillation to
% We now show
% our statistical view of distillation
% suggests 
% a novel application to 
%\XLC{} 
\emph{multiclass retrieval}.
% problems, 
%where a key challenge is selecting informative negatives during training.
Our basic idea is to 
%by 
% instruct the loss as to relative importance of competing labels.
% The resulting 
construct a
\emph{double-distillation} objective, 
wherein distillation informs the loss as to the relative confidence of both ``positive'' \emph{and} ``negative'' labels.
% an interesting interpretation of smoothing both positives \emph{and} negatives.
% We further show how distillation can be used to sample informative negatives during training.


%
\subsection{Double-distillation for multiclass retrieval}

Recall from~\eqref{eqn:top-k-risk}
that in multiclass retrieval,
we wish to ensure that the top-ranked labels in our predictor $f( x ) \in \Real^L$ contain the true label.
The softmax-cross entropy $\ell( y, f( x ) )$ in~\eqref{eqn:softmax-xent}
offers a reasonable surrogate loss for this task, since
$$ \lim_{\gamma \to 0} \frac{1}{\gamma} \cdot \log\left[ \sum_{y' \in [L]} e^{\gamma \cdot (f_{y'}( x ) - f_{y}( x ))} \right] = \max_{y' \neq y} f_{y'}( x ) - f_{y}( x ). $$
The latter is 
related to
the Cramer-Singer loss~\citep{Crammer:2002},
which bounds the top-$1$ retrieval loss.
Given a sample $\{ ( x_n, y_n ) \}_{n = 1}^N$,
we thus seek to minimise $\ell( y_n, f( x_n ) )$.
From our statistical view,
there is value in instead computing $\pStar( x_n )^{\tup} \ell( f( x_n ) )$:
intuitively,
each $y \in [L]$ acts a ``smooth positive'',
weighted by the Bayes probability $\pStar_y( x_n )$.

%
We observe,
however,
that such smoothing does \emph{not} affect the innards of the loss itself.
In particular,
one critique of~\eqref{eqn:softmax-xent} is that it assigns equal importance to each $y' \in [ L ]$.
% Intuitively, we would like to strongly penalise mistakes on labels that are clearly dissimilar from $y$.
Intuitively,
mistakes on labels $y'$ that are a \emph{poor} explanation for $x$ 
---
i.e., have \emph{low} $\pStar_{y'}( x )$
---
ought to be strongly penalised.
On the other hand, if under the Bayes probabilities some $y' \neq y$ strongly explains $x$,
it ought to be ignored.

To this end, 
consider a generalised softmax cross-entropy:
\begin{equation}
    \label{eqn:generalised-xent}
    \ell( y, f( x ) ) \defEq \log \E{\Y' \sim P( x )}{ e^{f_{\Y'}( \X ) - f_{y}( \X )} },
\end{equation}
where $P( x ) \in \Delta_L$ is a distribution over labels.
When $P( x )$ is uniform, this is exactly the standard cross-entropy loss~(cf.~\eqref{eqn:softmax-xent}) plus a constant.
For non-uniform $P( x )$, however, the loss 
%weighs individual labels $y'$ differently.
% This can be seen as encouraging that we \emph{rank} the labels according to their order in $P$.
%Thus, we 
is encouraged to focus on ensuring
$f_{y}( x ) \gg f_{y'}( x )$
for those $y'$ with large $P_{y'}( x )$. 
%$P_{y}( x ) \ll P_{y'}( x )$.

%
Continuing our statistical view, we posit that an ideal choice of $P$
is $P( x ) = \Psi( \pStar( x ) )$,
where $\Psi( \cdot )$ is some decreasing function.
% Our underlying risk is thus
% $$ R( f ) = \ES{\X}{ \ES{\Y \sim \pStar( \X )}{ \log\left[ \E{\Y' \sim (1 - \pStar( \X ))}{ e^{f_{\Y'}( \X ) - f_{y}( \X )} } \right]  } } $$
Concretely,
our new loss for a given $(x, y)$ is
$$ \ell( y, f( x ) ) = \log \sum_{y' \in [L]} \Psi( \pStar_{y'}( x ) ) \cdot e^{f_{y'}( x ) - f_{y}( x )}. $$
Intuitively, 
the loss treats $y$ as a ``positive'' label for $x$,
and each $y' \in [L]$ where $y' \neq y$ as a ``negative'' label.
% The scores $f_{y'}$ for these negatives are encouraged to be pushed below $f_y$,
% \emph{but} in a manner proportional to how well $y'$ describes $x$.
The loss seeks to score the positive label over 
\emph{all labels which poorly explain $x$}.
Compared to the standard softmax cross-entropy,
we avoid penalisation when $y'$ plausibly explains $x$ as well.

%
Recall that under a distillation setup, a teacher model provides us estimates $\pTeach( x )$ of $\pStar( x )$.
Consequently, 
to estimate this risk on a finite sample $S = \{ ( x_n, y_n ) \}_{n = 1}^N$,
we may construct
the following \emph{double-distillation} objective:
%\begin{tcolorbox}[boxsep=0pt,left=2pt,right=2pt,top=0pt,bottom=2pt,colback=black!5]
\begin{equation}
    \label{eqn:double-distillation}
    \begin{aligned}
    \RDist( f; S ) &= \frac{1}{N} \sum_{n = 1}^{N} \pTeach( x_n )^{\tup} \ell( f( x_n ) ) \\
    \ell( y, f( x_n ) ) &= \log \left[ \overline{\pTeach}( x_n )^{\tup} e^{f( x_n ) -  f_{y}( x_n )} \right],
    \end{aligned}
\end{equation}
%\end{tcolorbox}
where $\overline{\pTeach}( x ) \defEq \Psi( {\pTeach}( x ) )$;
% ARXIV
unrolling,
this corresponds to the objective
$$ \RDist( f; S ) = \frac{1}{N} \sum_{n = 1}^{N} \sum_{y \in [L]} \pTeach( y \mid x_n ) \cdot \log \left[ \sum_{y' \in [L]} \overline{\pTeach}( y' \mid x_n ) \cdot e^{f_{y'}( x_n ) -  f_{y}( x_n )} \right]. $$
Observe that~\eqref{eqn:double-distillation} uses the teacher in two ways: the first is the standard use of distillation to smooth the ``positive'' training labels.
% This effectively constructs an ``alternate positive'' for each $y \neq y_n$,
% weighted by the teacher confidence.
The second is a novel use of distillation to smooth the \emph{``negative''} labels.
Here, for any candidate ``positive'' label $y$,
we apply varying weights to ``negative'' labels $y' \neq y$
when computing 
% ARXIV
each
$\ell( y, f( x ) )$.
% We shall empirically verify the benefits of this negative smoothing in~\S\ref{sec:double-dist-expts}.


% %
% % \subsection{Negative mining via distillation}
% \subsection{Distillation meets \XLC{}}

% Further to the above,
% as a final remark we note that
% distillation also offers a means of solving a key challenge in \emph{\XLC{}} settings~\citep{Prabhu:2018,Jain:2019,Reddi:2019,Guo:2019}.
% The \XLC{} setting involves multiclass retrieval
% with a large number of classes $L$.
% A core challenge is being able to efficiently approximate the 
% loss function on a single sample,
% so that it does not require computing all $L$ scores.
% This is typically achieved by \emph{negative mining}~\citep{Sung:1996,Dalal:2005,Felzenszwalb:2010},
% which selects a subsample of labels
% on which to compute the loss.

% As a concrete example,
% observe that the generalised softmax cross-entropy loss~\eqref{eqn:generalised-xent} 
% may be approximated by
% $$ \hat{\ell}( y, f( x ) ) = \log \sum_{y' \in \hat{\YCal}} \frac{P_{y'}( x )}{Q_{y'}( x )} \cdot e^{f_{y'}( x ) - f_{y}( x )} $$
% for any distribution $Q( x ) \in \Delta_L$ over the labels,
% and
% $L' \ll L$ labels $\hat{\YCal}$ according to $Q( x )$.
% The inner sum approximates the full expectation by importance weighting.
% While transforming the result through the $\log$ is biased,
% this can be mitigated with suitable modelling~\citep{Bengio:2008,Jean:2015,Blanc:2018,Rawat:2019}.

% % is expressible as
% % \begin{align*}
% %     \ell( y, f( x ) ) %&= \log \E{\Y' \sim P( x )}{ e^{f_{\Y'}( \X ) - f_{y}( \X )} } \\
% %     &= \log \E{\Y' \sim Q( x )}{ \frac{P_{\Y'}( x )}{Q_{\Y'}( x )} \cdot e^{f_{\Y'}( x ) - f_{y}( x )} }.
% % \end{align*}
% % % Observe now that by the importance-weighting identity, 
% % for any distribution $Q( x ) \in \Delta_L$ over the labels.
% % The above is simply the importance weighting identity,
% % and amounts to a re-expression of the loss.
% % However, it suggests a means of approximating $\ell$ when $L$ is large:
% % we may draw $L' \ll L$ labels $\hat{\YCal}$ according to $Q( x )$, and use these to compute an empirical estimate for the expectation:
% % $$ \hat{\ell}( y, f( x ) ) = \log \sum_{y' \in \hat{\YCal}} \frac{P_{y'}( x )}{Q_{y'}( x )} \cdot e^{f_{y'}( x ) - f_{y}( x )}. $$
% % While the resulting estimate is biased for the softmax owing to the $\log$ transformation,
% % this can be mitigated with suitable modelling~\citep{Bengio:2008,Jean:2015,Blanc:2018,Rawat:2019}.

% %
% % In the above,
% % any valid distribution $Q( x )$ leads to an unbiased estimate.
% % However, different choices will affect the \emph{variance} of the estimates.
% % The choice which minimises the variance 
% The choice of $Q$ with minimal variance
% is $Q_{y'}( x ) \propto P_{y'}( x ) \cdot e^{f_{y'}( x )}$,
% so that the labels are sampled according to the current model scores.
% % This motivates, e.g., techniques such as the sampled softmax~\citep{Bengio:2008,Jean:2015,Grave:2017}.
% For the double-distillation objective~\eqref{eqn:double-distillation},
% %where $P( x ) = \overline{\pTeach}( x )$,
% our ideal sampling distribution is thus $Q_{y'}( x ) \propto \overline{\pTeach}( x ) \cdot e^{f_{y'}( x )}$.
% %The dependence on $f$ is undesirable, since it requires modifying our distribution at every iteration of training.
% %Suppose we replace these with the \emph{teacher's} scores,
% %so that 
% We may further approximate the second term with the teacher predictions, yielding
% $Q_{y'}( x ) \propto \overline{\pTeach}( x ) \cdot \pTeach( x )$.
% % This will be a reasonable approximation during later stages of student training,
% % when it has a reasonable model. 
% Intuitively, this will involve drawing as ``negatives'' those labels which 
% %the teacher believes to be the most plausible for the current instance $x$.
% \emph{maximally confuse the teacher}.
% % In practice, we may use a uniform $Q$ in early stages of training, and the above once the student starts to converge.

It remains to specify the precise form of $\Psi( \cdot )$ in~\eqref{eqn:double-distillation}.
A natural choice of $1 - \pTeach( x )$;
however, since the entries of $\pTeach( x )$ sum to one,
this may not allow the loss to sufficiently ignore other ``positive'' labels.
Concretely, suppose there are $L^+$ plausible ``positive'' labels,
which have most of the probability mass under $\pTeach( x )$.
Then, the total weight assigned to these labels will be roughly $L^+ - 1$;
this is of the order of $L^+$, which is what we would get from uniform weights.

% but since the entries of $\pTeach( x )$ sum to one,
% the scale of $\overline{\pTeach}( x )$ will be compressed.
To resolve this, we may instead use weights 
proportional to
$1 - \sigma( a \cdot s_{y}( x ) )$,
where $\sigma( \cdot )$ is the sigmoid function,
$s_y( x )$ is the teacher \emph{logit},
and $a > 0$ is a scaling parameter which may be tuned.
This parameterisation allows for multiple labels to have high (or low) weights.
In the above example,
each ``positive'' label can individually get a score close to $0$.
The total weight of the ``positives'' can thus also be close to $0$,
and so the loss can learn to ignore them.

%
\subsection{Discussion and implications}

The viability of distillation as a means of smoothing negatives has not, to our knowledge, been explored in the literature.
The proposal is, however, a natural consequence of our statistical view of distillation developed in~\S\ref{sec:analysis}.

The double-distillation objective in \eqref{eqn:double-distillation} relates to ranking losses.
In bipartite ranking settings~\citep{Cohen:1999},
one assumes an instance space $\XCal$ and binary labels $\YCal = \{ 0, 1 \}$ denoting that items are either relevant, or irrelevant.
\citet{Rudin:2009} proposed the following \emph{push loss} for this task:
\begin{align*}
    R_{\mathrm{push}}( h ) &\defEq \E{z \sim \Pr_{+}}{ g\left( \E{z' \sim \Pr_{-}}{ \phi( h( z' ) - h( z ) ) } \right) }
\end{align*}
where $\Pr_{+}$ and $\Pr_{-}$ are distributions over positive and negative instances respectively,
and $g( \cdot ), \phi( \cdot )$ are convex non-decreasing functions.
% $g( \cdot )$ is some convex non-decreasing function with large $g'( 0 )$,
% and $\phi( \cdot )$ is some convex non-increasing function.
Similar losses have also been studied in~\citet{Yun:2014}.
% When  and $\ell$ is the exponential loss,
% the objective is akin to the softmax cross-entropy.
The generalised softmax cross-entropy in~\eqref{eqn:generalised-xent}
can be seen as a \emph{contextual} version of this objective for each $x \in \XCal$,
where $g( z ) = \log( 1 + z )$ and $\phi( z ) = e^{-z}$.
In double-distillation, 
the contextual distributions $\Pr_{\pm}( x )$ are approximated using the teacher's predictions $\pTeach( x )$.
% In the present setup, we effectively treat both $\Pr_{\pm}$ as the distribution over labels produced by the teacher.
% \emph{However}, we additionally weigh the inner quantity by the inverse of the negative class-conditional density $\Pr_{-}$.

% ARXIV
There is a broad literature on using a weight on ``negatives'' in the softmax~\citep{Liu:2016,Liu:2017,Wang:2018,Li:2019,Cao:2019};
this is typically motivated by ensuring a varying margin for different classes.
The resulting weighting is thus either constant or label-dependent,
rather than the label- and example-dependent weights provided by distillation.
Closer still to our framework is the recent work of~\citet{Khan:2019},
which employs uncertainty estimates in the predictions for a given example and label to adjust the desired margin in the softmax.
While not explicitly couched in terms of distillation,
this may be understood as a ``self-distillation'' setup,
wherein the current predictions of a model are used to progressively refine future iterates.
Compared to double-distillation, however, the nature of the weighting employed is considerably more complicated.

% For example,~\citep{Liu:2016} propose the loss
% $$ \ell( y, f ) = \log\left[ 1 + \sum_{y' \neq y} e^{f_{y'} - \alpha_{y} \cdot f_{y}} \right], $$
% where $\alpha_{y}$ is some function of the angle between the example and weight vector for the $y$th class.

% While our discussion has focussed on the softmax cross-entropy,
% there are other proposals for \XLR{} wherein double-distillation may be useful.
% For example, consider the \emph{order-weighted losses}~\citet{Usunier:2009}
% \begin{equation}
%     \label{eqn:bowl}
%     \ell( y, f( x ) ) = \phi( f_y( x ) ) + \mathrm{avg}_{\mathrm{top}( k )}\left( \{ \phi( -f_{y'}( x ) ) \}_{y' \neq y} \right),
% \end{equation}
% where 
% $\phi \colon \Real \to \Real_+$ is a margin loss,
% $k$ is an integer,
% and $\mathrm{avg}_{\mathrm{top}( k )}$ denotes the average of the top-$k$ largest elements of a vector.
% \citet{Reddi:2019} proposed a means of efficiently optimising such losses,
% wherein the second term is computed over a random sample of labels.
% Following the above, one may both 
% perform a \emph{weighted} average and sample these labels according to a teacher distribution.

There is a rich literature on the problem of label ranking,
where typically it is assumed that one observes a (partial) ground-truth ranking over labels~\citep{Dekel:2004,Furnkranz:2008,Vembu:2011}.
We remark also that the 
%ranking loss 
view of
the softmax as a ranking loss has received recent attention~\citep{Bruch:2019,Bruch:2019b}.
Exploiting the statistical view of distillation in these regimes is a promising future direction.
%
\citet{Tang:2018} explored distillation in a related learning-to-rank framework.
While similar in spirit,
this focusses on pointwise losses, 
wherein the distinction between positive and negative smoothing is absent.

Finally, we note that while our discussion has focussed on the softmax cross-entropy,
double-distillation may be useful for a broader class of losses,
e.g.,
\emph{order-weighted losses} as explored in~\citet{Usunier:2009,Reddi:2019}.

% This can be generalised to the family of binary order weighted losses~\citep{Usunier:2009,Reddi:2019},
% $$ \ell( y, f( x ) ) \defEq \phi( f_{y}( x ) ) + \mathrm{owa}( \{ \phi( -f_{y'}( x ) ) \mid y' \neq y \}; \theta ), $$
% where $\mathrm{owa}( \cdot; \theta )$ is an order-weighted average with weights $\theta$.
% Observe that for the standard unweighted average, we obtain the loss
% \begin{align*}
%     \ell( y, f( x ) ) &\defEq \phi( f_{y}( x ) ) + \sum_{y' \neq y} \phi( -f_{y'}( x ) ) \\
%     &= \phi( f_{y}( x ) ) - \phi( -f_{y}( x ) ) + \\
%     &\E{\Y' \sim Q( x )}{ \frac{1}{q_{\Y'}( x )} \cdot \phi( -f_{\Y'}( x ) ) },
% \end{align*}
% where as before $Q( x )$ is some distribution over the labels.
% \log \underset{\mathsf{Y'} \sim P}{\mathbb{E}}\left[ e^{f_{\mathsf{Y}'} - f_y{}} \right] = \log \underset{\mathsf{Y'} \sim Q}{\mathbb{E}}\left[ \frac{P( \mathsf{Y'} )}{Q( \mathsf{Y'} )} \cdot e^{f_{\mathsf{Y}'} - f_y{}} \right]
% %\log \underset{\mathsf{Y'} \sim \mathrm{Uni}}{\mathbb{E}}\left[ e^{f_{\mathsf{Y}'} - f_y{}} \right] = \log \underset{\mathsf{Y'} \sim Q}{\mathbb{E}}\left[ \frac{1}{Q( \mathsf{Y}' )} \cdot e^{f_{\mathsf{Y}'} - f_y{}} \right]
% For the one-versus-all loss, we obtain
% \begin{align*}
%     \bar{\ell}( y, f( x ) ) &\defEq \phi( f_{y}( x ) ) - \phi( -f_{y}( x ) ) + \\
%     &\frac{1}{L - 1} \cdot \sum_{y' \in \bar{\YCal}} \frac{1}{q_{y'}( x )} \cdot \phi( -f_{y'}( x ) ).
% \end{align*}

% Now suppose that the student has a reasonable model,
% so that $e^{f_y( x )} \sim \pStar( x )$.
% Since the teacher model already provides us 
% Consequently, given a teacher model's estimates of these probabilities, we propose to 
% use 
% plug them in as our $Q( x )$,
% i.e.,
% use $q_{y'}( x ) \propto e^{f^{\mathrm{teach}}_{y'}( x )}$.
% Picking $q_{y'}( x ) \propto \phi(- {f^{\mathrm{teach}}_{y'}( x )} )$ will pick labels that incur a high loss according to the teacher's predictions,
% i.e.,
% which the teacher deemed most likely to be positive.
% Having drawn some samples from this distribution, one may apply the order weighted average as before.

% %
% \subsection{The double-distillation objective}

% Putting the above together, we arrive at the following
% \emph{double-distillation} objective
% for a training sample $S$
% and the softmax cross-entropy loss:
% \begin{align*}
% R_{\mathrm{ddist}}( f; S ) &= \frac{1}{N} \sum_{n \in [N]} \E{\Y \sim \hat{p}( x_n )}{ \log \Delta( x_n, \Y )  } \\
% \Delta( x_n, y ) &\defEq \E{\Y' \sim q( x_n )}{ \frac{1}{q_{\Y'}( x_n )} \cdot e^{f_{\Y'}( x_n) - f_{y}( x_n )} },
% \end{align*}
% where $\hat{p}$ are the predictions given by the teacher,
% and
% $q$ are the exponents of the predictions given by the teacher.

% Similarly,
% for a BOWL loss,
% we have
% \begin{align*}
% R_{\mathrm{ddist}}( f; S ) &= \frac{1}{N} \sum_{n \in [N]} \E{\Y \sim \hat{p}( x_n )}{ \phi( f_{\Y}( x_n ) ) - \phi( -f_{\Y}( x_n ) ) } + \\
% &\E{\Y' \sim q( x_n )}{ \frac{1}{q_{\Y'}( x_n )} \cdot \phi( -f_{\Y'}( x_n ) ) }.
% \end{align*}
% Observe that when $q$ is a uniform distribution, this corresponds to stochastic negative mining~\citep{Reddi:2019}.
% Further, when $\hat{p} = q$, then 
% %\ankit{Why is the following true? Can we replace $Y' = Y$?}
% \begin{align*}
% R_{\mathrm{ddist}}( f; S ) &= \frac{1}{N} \sum_{n \in [N]} \E{\Y \sim \hat{p}( x_n )}{ \bar{\ell}( x_n, \Y; f ) } \\
% \bar{\ell}( x_n, y; f ) &\defEq \phi( f_{y}( x_n ) ) + \left( \frac{1}{\hat{p}_y( x_n )} - 1 \right) \cdot \phi( -f_{y}( x_n ) ).
% \end{align*}
% This loss is intuitive: when $\hat{p}_y( x_n ) \ll 1$, so that the teacher believes that label $y$ is not a good fit for $x_n$, then we {\color{red} upweight} the negative loss component.
% On the other hand,
% when $\hat{p}_y( x_n ) \gg 1$ {\color{red}??$\hat{p}_y( x_n ) \approx 1$??}, so that the teacher believes that label $y$ is a good fit for $x_n$, then we upweight the positive loss component.

% {\bf\color{red} TODO: integrate top-$k$ here. sparsify the teacher distribution for the negatives?}

==> Why distillation helps ICML 2020/experiments.tex <==
We now present experiments illustrating three key points:
\begin{enumerate}[label=(\roman*),itemsep=0pt,topsep=0pt]
    \item we show that distilling with true (Bayes) class-probabilities improves generalisation over one-hot labels,
    validating
    our statistical view of distillation.

    \item we illustrate our bias-variance tradeoff on synthetic and real-world datasets,
    confirming that teachers with good estimates of $\pStar$ can be usefully distilled.

    \item we finally show that double-distillation performs well on real-world multiclass retrieval datasets,
    confirming the broader value in our statistical perspective.
%yielding an approach with superior performance and training efficiency over the current state-of-the-art.
\end{enumerate}


%
\begin{figure*}[!t]
    \centering
    
    %\begin{minipage}[t][][t]{0.475\linewidth}
    \subfigure[Student AUC versus \# of training samples.]{
    \includegraphics[scale=0.4,valign=t]{figs/gaussian_distillation.pdf}
%     \caption{Distillation versus one-hot encoding on a synthetic dataset comprising Gaussian class-conditionals, as the number of training samples is varied.
% We observe two key trends:
% first, distillation generally offers a noticeable gain over the standard one-hot encoding.
% Second, both methods see improved performance with more samples, but the gains are greater for the one-hot encoding.}
    \label{fig:gaussian_distillation}
    }
%\end{figure*}
    %\end{minipage}%
%
%\begin{figure*}
    %\centering
    \qquad%
    %\begin{minipage}[t][][t]{0.475\linewidth}
    \subfigure[Student AUC versus class separation.]{
    \includegraphics[scale=0.4,valign=t]{figs/gaussian_distillation_vs_r.pdf}
%     \caption{Distillation versus one-hot encoding on a synthetic dataset comprising Gaussian class-conditionals, as the norm $r$ of the class-conditional centroids is varied.
% Both methods see worse performance as $r$ is smaller, but the gains of distillation over the one-hot encoding are greater for this setting.}
    \label{fig:gaussian_distillation_vs_r}
    }
    %\end{minipage}
    
    \caption{Distillation with Bayes-teacher on synthetic data comprising Gaussian class-conditionals.
Distillation offers a noticeable gain over the standard one-hot encoding,
particularly in the small-sample regime (left),
and when the underlying problem is noisier (right).
    }
\end{figure*}

% %
% \begin{figure*}[!t]
%     \centering
    
%     \subfigure[Synthetic dataset.]{
%     \includegraphics[scale=0.4]{figs/gaussian_distillation_bias_variance.pdf}
%     \label{fig:gaussian_distillation_bias_variance}
%     }%
%     \subfigure[Fashion MNIST dataset.]{
%     \includegraphics[scale=0.4]{figs/fmnist_distillation_bias_variance.pdf}
%     \label{fig:fmnist_distillation_bias_variance}
%     }    

%     \caption{Relationship between teacher's MSE against true class-probability and student's test set AUC.
%     As predicted by the theory, teachers which better approximate $\pStar$ yield better students.}
% \end{figure*}

%
\subsection{Is Bayes a good teacher for distillation?}
\label{sec:experiments-bayes}

To illustrate our statistical perspective, we conduct a synthetic experiment where $\pStar( x )$ is known,
and show that distilling these Bayes class-probabilities benefits learning.

We generate training samples $S = \{ ( x_n, y_n ) \}_{i = 1}^N$ from a distribution $\Pr$ comprising class-conditionals which are each 10-dimensional Gaussians,
with means $\pm ( 1, 1, \ldots, 1 )$ respectively.
By construction, 
the Bayes class-probability distribution is 
$\pStar( x ) = ( \Pr( y = 0 \mid x ), \Pr( y = 1 \mid x ) )$
where
$\Pr( y = 1 \mid x ) = \sigma( (\theta^*)^{\tup}  x ) $,
for $\theta^* \defEq ( 2, 2, \ldots, 2 )$.

We compare two training procedures:
standard logistic regression on $S$, 
and \emph{Bayes-distilled} logistic regression using $\pStar( x_n )$ per~\eqref{eqn:bayes-distillation}.
%(with the standard one-hot encoding of labels),
%and the other which employs a \emph{weighted} logistic regression on the 
%\emph{Bayes-distilled} samples $S' = \{ ( x_n, +1 ) \}_{i = 1}^N \cup \{ ( x_n, -1 ) \}_{i = 1}^N$, 
%where $(x_n, +1)$ has weight 
%$w_i \defEq \sigma( (\theta^*)^{\tup}  x  )$.
%$\pStar( x_n )$
%and $(x_n, -1)$ has weight $1 - \pStar( x_n )$.
% Note that $w_i$ thus corresponds to the true class-conditional density ratio $\frac{p_+(x_n)}{p_-(x_n)}$.
Logistic regression is well-specified for this problem,
i.e.,
as $N \to \infty$,
the standard learner will learn $\theta^*$.
However, 
we will demonstrate
that on finite samples,
the Bayes-distilled learner's knowledge of $\pStar( x_n )$ will be beneficial.
We reiterate that while this learner could trivially memorise the training $\pStar( x_n )$,
this would not generalise.

Figure~\ref{fig:gaussian_distillation} compares the performance of these two approaches for varying training set sizes, where for each training set size we perform $100$ independent trials and measure the AUC-ROC on a test set of $10^4$ samples.
We observe two key trends:
first, Bayes-distillation generally offers a noticeable gain over the standard one-hot encoding,
in line with our theoretical guarantee of low variance.

Second, both methods see improved performance with more samples, but the gains are greater for the one-hot encoding.
This in line with our intuition that distillation effectively augments each training sample:
when $N$ is large to begin with, the marginal gain of such augmentation is minimal.

Figure~\ref{fig:gaussian_distillation_vs_r} continues the exploration of this setting.
We now vary the distance $r$ between the means of each of the Gaussians.
% by now scaling the class-conditional means by some $r > 0$.
When $r$ is small, the two distributions grow closer together, making the classification problem more challenging.
We thus observe that both methods see worse performance as $r$ is smaller.
At the same time, smaller $r$ makes the one-hot labels have higher variance compared to the Bayes class-probabilities.
Consequently, the gains of distillation over the one-hot encoding are greater for this setting,
in line with our guarantee on the lower-variance Bayes-distilled risk aiding generalisation (Proposition~\ref{prop:svp}).
%This is in line with our theoretical guarantee on distillation improving generalisation when the underlying Bayes error is large.

As a final experiment, we verify the claim that teacher accuracy does \emph{not} suffice for improving student generalisation,
since this does not necessarily correlate with the quality of the teacher's probability estimates.
We assess this by artificially distorting the teacher probabilities so as to perfectly preserve teacher accuracy,
while degrading their approximation to $\pStar$.
Appendix~\ref{sec:distorted_bayes_distillation} presents plots confirming that such degradation progressively reduces the gains of distillation.


%
\subsection{Illustration of bias-variance tradeoff}

We next illustrate our analysis 
on the bias-variance tradeoff in distillation
from~\S\ref{sec:bias-variance} on {synthetic and real-world} datasets.

%
\textbf{Synthetic}.
% Continuing the same synthetic Gaussian data as above,
We now train a series of increasingly complex teacher models $\pTeach$,
and assess their resulting distillation benefit on a synthetic problem.
Here, the data is sampled from a marginal $\Pr( x )$ which is a zero-mean isotropic Gaussian in 2D.
The class-probability function is given by $\eta( x ) = \sigma( 2 \cdot (\| x \|_{\infty} - 0.5) )$, so that the negatives are concentrated in a rectangular slab.

We consider teachers that are 
%decision trees of 
random forests of
a fixed depth $d \in \{ 1, 2, 4, 8, 16 \}$, with $3$ base estimators.
Increasing $d$ has the effect of reducing teacher \emph{bias} (since the class of depth-$d$ trees can better approximate $\pStar$),
but increasing teacher \emph{variance} (since the class of depth-$d$ trees can induce complex decision boundaries).
For fixed $d$, we train a teacher model on the given training sample $S$ (with $N = 100$).
%per the previous section.
We then distill the teacher predictions to a student model, which is a depth $4$ tree.
% As before, the logistic regression model is well-specified, but one can hope for better generalisation via instructive teacher probabilities on noisy samples.
For each such teacher, we compute its MSE,
as well as the test set AUC of the corresponding distilled student.
We repeat this for $100$ independent trials.

Figure~\ref{fig:gaussian_distillation_tree_depth_vs_mse} and~\ref{fig:gaussian_distillation_tree_depth_vs_auc}
show how the teacher's depth affects its MSE in modelling $\pStar$, as well as the AUC of the resulting distilled student.
There is an optimal depth $d = 8$ at which the teacher achieves the best MSE approximation of $\pStar$.
In keeping with the theory, this also corresponds to the teacher whose resulting student generalises the best.
Figure~\ref{fig:gaussian_distillation_tree_bias_variance} combines these plots to explicitly show the relationship between the the teacher's MSE and the student's AUC.
In line with the theory, more accurate estimates of $\pStar$ result in better students.

Note that at depth $10$, the teacher model is expected to have lower bias;
however, it results in a slightly worse distilled student.
This verifies that \emph{one may favour a higher-bias teacher}
\emph{if it has lower variance}: a teacher may achieve a lower MSE -- and thus distill better -- by slightly increasing its bias while lowering variance. See Appendix~\ref{app:experiments-bias-variance} for additional bias-variance experiments on synthetic data.

%
\textbf{Fashion MNIST}.
It is challenging to assess the bias-variance tradeoff on real-world datasets,
where the Bayes $\pStar( x )$ is unknown.
% Nonetheless, we examine the effect of introducing bias and variance into a powerful teacher model.
As a proxy, 
we take the fashion MNIST dataset,
and treat a powerful teacher model as our $\pStar$.
We train an MLP teacher with two hidden layers with $128$ and $10$ dimensions. %, and ReLU and sigmoid activations respectively.
This achieves a test accuracy of $\sim 89\%$.

We then inject bias and noise per~\eqref{eqn:noisy-bayes},
and distill the result to a linear logistic regression model.
To amplify the effects of distillation, we constrain the student by only offering it the top $2500$ samples that the original teacher deems most uncertain.
Figures~\ref{fig:fmnist_distillation_bias_variance} %and~\ref{fig:fmnist_distillation_bias_variance_mse}
demonstrates similar trend to the synthetic dataset,
with the best MSE approximator to the original teacher generally yielding the best student.


%
\textbf{CIFAR-100}.
\label{sec:bias-variance-cifar100}
We verify that accurate probabilty estimation by the teacher strongly influences student generalisation, and that this can be at odds with accuracy.
We revisit the plots introduced in Figure~\ref{fig:cifar100-distillation}.
Here, we train ResNets of varying depths on the CIFAR-100 dataset,
and use these as teachers to distill to a student ResNet of fixed depth $8$.
Figure~\ref{fig:cifar100_acc} reveals that the teacher model gets increasingly more accurate as its depth increases;
\emph{however}, the corresponding log-loss %and calibration error 
starts increasing beyond a depth of $14$.
This indicates the teacher's probability estimates become progressively poorer approximations of the Bayes class-probability distribution $\pStar( x )$. The accuracy of the student model also degrades beyond a teacher depth of $14$, reflecting the bias-variance bound in Proposition~\ref{prop:bias-variance}.

% %
% \begin{figure}[!t]
%     \centering
    
%     \subfigure[Synthetic dataset.]{
%     \includegraphics[scale=0.26]{figs/gaussian_distillation_bias_variance.pdf}
%     \label{fig:gaussian_distillation_bias_variance}
%     }%
%     \subfigure[Fashion MNIST dataset.]{
%     \includegraphics[scale=0.26]{figs/fmnist_distillation_bias_variance.pdf}
%     \label{fig:fmnist_distillation_bias_variance}
%     }    

%     \caption{Relationship between teacher's MSE against true class-probability and student's test set AUC.
%     As predicted by the theory, teachers which better approximate $\pStar$ yield better students.}
% \end{figure}

%
\begin{figure}[!t]
    \centering
    
    \subfigure[Teacher depth versus MSE.]{
    \includegraphics[scale=0.47]{figs/distillation_tree_depth_vs_mse_v3.pdf}
    \label{fig:gaussian_distillation_tree_depth_vs_mse}
    }%
    \subfigure[Teacher depth versus student AUC.]{
    \includegraphics[scale=0.47]{figs/distillation_tree_depth_vs_auc_v3.pdf}
    \label{fig:gaussian_distillation_tree_depth_vs_auc}
    }    

    \caption{Relationship between depth of teacher's decision tree model (model complexity) and its MSE in modelling $\pStar$, as well as the AUC of the resulting distilled student, on a synthetic 
    %Gaussian problem of~\S\ref{sec:experiments-bayes}.
    problem.
    There is an optimal depth $d = 8$ at which the teacher achieves the best MSE approximation of $\pStar$.
    In keeping with the theory, 
    this corresponds to the teacher whose resulting student generalises the best.}
\end{figure}

% ARXIV
\begin{figure}[!t]
    \centering
    
    \subfigure[Synthetic dataset.]{
    \includegraphics[scale=0.47]{figs/distillation_tree_mse_vs_auc.pdf}
    \label{fig:gaussian_distillation_tree_bias_variance}
    }%
    \subfigure[Fashion MNIST dataset.]{
    \includegraphics[scale=0.47]{figs/fmnist_distillation_bias_variance.pdf}
    \label{fig:fmnist_distillation_bias_variance}
    }    

    \caption{Relationship between teacher's MSE against true class-probability and student's test set AUC.
    In keeping with the theory, teachers which better approximate $\pStar$ in an MSE sense
    yield better students.}
\end{figure}


%
\subsection{Double-distillation for \XLR{}}
\label{sec:double-dist-expts}

Our final set of experiments confirm the value in our double-distillation objective in~\eqref{eqn:double-distillation}.
To do so, we use  the
{\sc AmazonCat-13K} and {\sc Amazon-670K}
 benchmark datasets for \XLR{}~\citep{McAuley:2013, Bhatia:2015}.
The data is multi\emph{label};
following~\citet{Reddi:2019}, we make it multiclass by
creating a single example $(x, y)$ for each label $y$ associated with $x$.

We construct a ``teacher'' model using a feedforward network with a single (linear) hidden layer of width $512$,
trained to minimise the softmax cross-entropy loss.
We then construct a ``student'' model using the same architecture, but with a hidden layer of width $8$ for {\sc AmazonCat-13K} and $64$ for {\sc Amazon-670K}
because  {\sc Amazon-670K} is significantly larger than {\sc AmazonCat-13K} (670k vs 13k labels).
This student model is compared to a distilled student,
where the teacher logits are used in place of the one-hot training labels.
Both methods are then compared to the double-distillation objective,
where the teacher logits are used to smooth the negatives in the softmax per~\eqref{eqn:generalised-xent} and~\eqref{eqn:double-distillation}.

We compare all methods using
the precision@$k$ metric
with $k \in \{ 1, 3, 5 \}$,
averaging these over multiple runs.
Table~\ref{tbl:double-distillation} summarises our findings.
% The reported numbers are the average of multiple runs.
We see that distillation offers a small but consistent bump in performance over the student baseline.
Double-distillation further improves upon this,
especially at the head of the prediction (P@1 and P@3),
confirming the value of weighing negatives differently.
The gains are particularly significant on {\sc AmazonCat-13K},
where the double-distilled student can \emph{improve} upon the teacher model itself.
Overall, our findings illustrate the broader value of the statistical perspective of distillation.


%
\begin{table*}[t!]
    \centering
    
    \begin{minipage}[t]{.475\linewidth}
    \begin{tabular}{@{}llll@{}}
        \toprule
        {\bf Method}                  & {\bf P@1} & {\bf P@3} & {\bf P@5} \\
        \toprule
        Teacher                       & 0.8495 & 0.7412 & 0.6109 \\
        \midrule
        Student                       & 0.7913 & 0.6156 & 0.4774 \\
        Student + distillation        & 0.8131 & 0.6363 & 0.4918 \\
        Student + double-distillation & \bf 0.8560 & \bf 0.7148 & \bf 0.5715 \\
        \bottomrule
    \end{tabular}
    %\caption{{\sc AmazonCat-13K}}
    
    \end{minipage}
    
    \qquad
    % ARXIV
    \vspace{\baselineskip}
    
    \begin{minipage}[t]{.475\linewidth}
    \begin{tabular}{@{}llll@{}}
        \toprule
        {\bf Method}                  & {\bf P@1} & {\bf P@3} & {\bf P@5} \\
        \toprule
        Teacher                       &  0.3983 &  0.3598 & 0.3298 \\
        \midrule
        Student                       &  0.3307 &  0.3004 & 0.2753 \\
        Student + distillation        &  0.3461 &  0.3151 & \bf 0.2892 \\
        Student + double-distillation &  \bf 0.3480 &  \bf 0.3161 & 0.2865 \\
        \bottomrule
    \end{tabular}
    
    %\caption{{\sc AmazonCat-670K}}
    \end{minipage}
    
    \caption{Precision@$k$ metrics for double-distillation objective against standard distillation and student baseline on {\sc AmazonCat-13K} (left) and {\sc AmazonCat-670K} (right).
    With double-distillation, the student is seen to significantly improve performance over training with one-hot labels, 
    but also a distilled model which applies uniform weighting of all negatives.
    }
    \label{tbl:double-distillation}
\end{table*}

% %
% \begin{table}[t!]
%     \centering
    
%     \resizebox{0.9\linewidth}{!}{
%     \begin{tabular}{@{}llll@{}}
%         \toprule
%         {\bf Method}                  & {\bf P@1} & {\bf P@3} & {\bf P@5} \\
%         \toprule
%         Teacher                       & 0.8495 & 0.7412 & 0.6109 \\
%         \midrule
%         Student                       & 0.7913 & 0.6156 & 0.4774 \\
%         Student + distillation        & 0.8131 & 0.6363 & 0.4918 \\
%         Student + double-distillation & \bf 0.8560 & \bf 0.7148 & \bf 0.5715 \\
%         \bottomrule
%     \end{tabular}
%     }
    
%     \caption{Precision@$k$ metrics for double-distillation objective against standard distillation and student baseline on {\sc AmazonCat-13K}.
%     With double-distillation, the student is seen to significantly improve performance over training with one-hot labels, 
%     but also a distilled model which applies uniform weighting of all negatives.
%     }
%     \label{tbl:double-distillation-amazoncat13k}
% \end{table}

% %
% \begin{table}[t!]
%     \centering
    
%     \resizebox{0.9\linewidth}{!}{
%     \begin{tabular}{@{}llll@{}}
%         \toprule
%         {\bf Method}                  & {\bf P@1} & {\bf P@3} & {\bf P@5} \\
%         \toprule
%         Teacher                       &  0.3983 &  0.3598 & 0.3298 \\
%         \midrule
%         Student                       &  0.3307 &  0.3004 & 0.2753 \\
%         Student + distillation        &  0.3461 &  0.3151 & \bf 0.2892 \\
%         Student + double-distillation &  \bf 0.3480 &  \bf 0.3161 & 0.2865 \\
%         \bottomrule
%     \end{tabular}
%     }
    
%     \caption{Precision@$k$ metrics for double-distillation objective against standard distillation and student baseline on~{\sc Amazon-670K}.
%     With double-distillation, the student is seen to improve performance in the top predictions (P@1 and P@3).
%     }
%     \label{tbl:double-distillation-amazon670k}
% \end{table}


==> Why distillation helps ICML 2020/intro.tex <==
Distillation is the process of using a ``teacher'' model to improve the performance of a ``student'' model~\citep{Craven:1995,Breiman:1996,Bucilua:2006,Xue:2013,Ba:2014,Hinton:2015}.
In its simplest form, 
rather than fitting to raw labels,
one trains the student to fit the teacher's \emph{distribution} over labels.
While originally devised with the aim of model compression, 
distillation has proven successful 
in iteratively improving a fixed-capacity model
%even when the student and teacher have the same capacity
~\citep{Rusu:2016,Furlanello:2018,Yang:2019,Xie:2019},
and found use in many other settings~\citep{Papernot:2016,Tang:2016,Czarnecki:2017,Celik:2017,Yim:2017,Li:2018,Liu:2019,Nayak:2019}.

Given its empirical successes, it is natural to ask: why does distillation help?
%Surprisingly, a clear answer to this question remains elusive.
\citet{Hinton:2015} argued that
distillation provides 
``dark knowledge'' via
teacher logits on 
%labels other than the training label,
the ``wrong'' labels $y' \neq y$ for an example $(x, y)$,
which effectively weights samples differently~\citep{Furlanello:2018}.
% While intuitive, to our knowledge, a precise statement of the benefits of this effect is lacking.
Various theoretical analyses of distillation have subsequently been developed~\citep{Lopez-Paz:2016,Phuong:2019,Foster:2019,Dong:2019,Mobahi:2020},
with particular focus on its optimisation and regularisation effects.
% but 
% a complete picture of its value remains elusive
%typically under restricted settings (see~\S\ref{sec:background-distillation}).
% A broader understanding of distillation is, to our knowledge, lacking.
%Besides being conceptually unsatisfying, 
%the incomplete understanding of distillation's success
%limits its broader use in other settings.
% The statistical effects of distillation have however received less attention.

In this paper,
we present a 
novel
statistical perspective on distillation
which sheds light on why it aids performance.
% and suggests an application to a novel setting.
Our analysis
centers on a simple observation:
%\emph{the teacher's label probabilities are estimates of the true} (Bayes-optimal) \emph{class-probabilities}.
\emph{a good teacher accurately models the true} (Bayes) \emph{class-probabilities}.
This is a stricter requirement than the teacher merely having high \emph{accuracy}.
% Motivated by this,
We quantify how 
%access to
such probability estimates 
improve generalisation
compared to
learning from raw labels.
Building on this,
we show how
distillation 
is also useful
in 
%\emph{selecting informative ``negatives''}
selecting \emph{informative labels}
for
multiclass \emph{retrieval},
wherein we wish to 
% which seeks to
order labels according to their relevance~\citep{Jain:2019}.
In sum, our contributions are:
\begin{enumerate}[label=(\roman*),itemsep=0pt,topsep=0pt]
    \item We establish the statistical benefit of using the Bayes class-probabilities in place of one-hot labels,
    and quantify a \emph{bias-variance} tradeoff
    when using approximate class-probabilities (\S\ref{sec:analysis}).

    \item We
    propose \emph{double-distillation}, 
    a novel application of distillation
    for
    \XLR{}
    wherein
    %smoothing is applied to both
    %the positive \emph{and} negative labels
    %smoothing is applied in two distinct forms
    teacher probabilities guide a \emph{ranking} over labels
    (\S\ref{sec:double_distillation}).

    \item We experimentally validate 
    the value of both approximate class-probabilities in terms of generalisation,
    and of
    double-distillation
    in multiclass \emph{retrieval} (\S\ref{sec:experiments}).
\end{enumerate}
Contribution (i) gives a statistical perspective 
on the value of
``dark knowledge'': 
for an example $(x, y)$,
the logits on ``wrong'' labels $y' \neq y$ 
encode information about the underlying 
% class-probability function.
data distribution.
% This information can be significantly more beneficial than raw labels,
% provided they have reasonable fidelity.
%Our bias-variance result 
This view elucidates
%when and how teacher probabilities can improve a student's generalisation;
how
a teacher's \emph{probability calibration}
rather than \emph{accuracy}
can influence a student's generalisation;
see Figure~\ref{fig:cifar100-distillation} for an illustration.
Contribution (ii) shows 
a practical benefit of
this statistical view %for 
%\XLC{},
%\XLR{},
%and exploiting it 
of distillation,
by showing how \XLR{} objectives benefit from approximate class-probabilities.

% %
% \begin{figure*}[!t]
%     \centering
    
%     \subfigure[Top-1 accuracy.]{
%     \includegraphics[scale=0.35]{figs/cifar100_top1_acc.pdf}
%     \label{fig:cifar100_acc}
%     }%
%     \subfigure[Log-loss.]{
%     \includegraphics[scale=0.35]{figs/cifar100_kl.pdf}
%     \label{fig:cifar100_kl}
%     }  
%     \subfigure[Expected calibration error.]{
%     \includegraphics[scale=0.35]{figs/cifar100_ece.pdf}
%     \label{fig:cifar100_ece}
%     } 
%     \caption{Illustration of 
%     %the  bias-variance tradeoff for distillation.
%     how better teacher modelling of underlying (Bayes) class-probabilities
%     influences student generalisation,
%     per our statistical perspective.
%     Here, we train ResNets of varying depths on the CIFAR-100 dataset,
%     and use these as teachers to distill to a student ResNet of fixed depth $8$.
%     Figure~\ref{fig:cifar100_acc} reveals that the teacher model gets increasingly more accurate as its depth increases;
%     \emph{however}, from~\ref{fig:cifar100_kl} 
%     the corresponding log-loss %and calibration error 
%     starts increasing beyond a depth of $14$.
%     The calibration error is also seen to worsen in ~\ref{fig:cifar100_ece}.
%     This indicates the teacher's probability estimates become progressively poorer approximations of the Bayes class-probability distribution $\pStar( x )$ after certain depth,
%     i.e., the teacher induces a higher bias.
%     The accuracy of the student model also degrades beyond a teacher depth of $14$, reflecting the bias-variance bound in Proposition~\ref{prop:bias-variance}.
%     See~\S\ref{sec:bias-variance-cifar100} for more details,
%     and~\S\ref{sec:bias-variance} for illustration of a general bias-variance tradeoff.
%     }
%     \label{fig:cifar100-distillation}
% \end{figure*}

% ARXIV
%
\begin{figure*}[!t]
    \centering
    
    \subfigure[Top-1 accuracy.]{
    \includegraphics[scale=0.45]{figs/cifar100_top1_acc.pdf}
    \label{fig:cifar100_acc}
    }%
    \subfigure[Log-loss.]{
    \includegraphics[scale=0.45]{figs/cifar100_kl.pdf}
    \label{fig:cifar100_kl}
    }  
    \subfigure[Expected calibration error.]{
    \includegraphics[scale=0.45]{figs/cifar100_ece.pdf}
    \label{fig:cifar100_ece}
    } 
    \caption{Illustration of 
    %the  bias-variance tradeoff for distillation.
    how better teacher modelling of underlying (Bayes) class-probabilities
    influences student generalisation,
    per our statistical perspective.
    Here, we train ResNets of varying depths on the CIFAR-100 dataset,
    and use these as teachers to distill to a student ResNet of fixed depth $8$.
    Figure~\ref{fig:cifar100_acc} reveals that the teacher model gets increasingly more accurate as its depth increases;
    \emph{however}, from~\ref{fig:cifar100_kl} 
    the corresponding log-loss
    starts increasing beyond a depth of $14$.
    The calibration error is also seen to worsen with increasing depth in~\ref{fig:cifar100_ece}.
    This indicates the teacher's probability estimates become progressively poorer approximations of the Bayes class-probability distribution $\pStar( x )$ after certain depth. Intuitively, the teacher's approximation of $\pStar$ is governed by balancing the bias and variance in its predictions.
    The accuracy of the student model also degrades beyond a teacher depth of $14$, reflecting the bound in Proposition~\ref{prop:bias-variance}. See~\S\ref{sec:bias-variance-cifar100} for more details,
    and~\S\ref{sec:bias-variance} for illustration of a general bias-variance tradeoff.
    }
    \label{fig:cifar100-distillation}
\end{figure*}


==> Why distillation helps ICML 2020/macros.tex <==
% !TEX root=./double_distillation.tex

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{natbib}

\usepackage{float}
\usepackage{graphicx}
\usepackage[export]{adjustbox}
\usepackage[inline]{enumitem}

\usepackage{amsmath,amssymb,amsthm}
\usepackage[mathscr]{eucal}
\usepackage{stmaryrd}
\usepackage{accents}
\usepackage{upgreek}

\usepackage[most]{tcolorbox}
\usepackage{setspace}

\usepackage{booktabs,colortbl,multirow}

\usepackage{algorithm,algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\usepackage{soul}

%
\newcommand{\XLC}{extreme classification}
\newcommand{\XLR}{multiclass retrieval}
\newcommand{\pStar}{p^*}
\newcommand{\pTeach}{{p}^{\mathrm{t}}}
\newcommand{\REmp}{\hat{R}}
\newcommand{\RDist}{\tilde{R}}
\newcommand{\RDistBayes}{\hat{R}_*}


%%%%%%%%%%%%%%%%%%%%%
\newcommand*\widefbox[1]{\fbox{\hspace{0.8em}#1\hspace{0.8em}}}

\graphicspath{{figs//}}

\allowdisplaybreaks

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

%%%

\newcommand{\eg}{e.g.\ }
\newcommand{\ie}{i.e.\ }

\newcommand{\edit}[2]{{\color{red}\st{#1}} {\color{ForestGreen}#2}}
\newcommand{\newedit}[1]{{\color{ForestGreen}#1}}

%

\newcommand{\Equation}[1]{Equation \ref{#1}}

\newcommand{\defEq}{\stackrel{.}{=}}

\newcommand{\indicator}[1]{\llbracket #1 \rrbracket}
\newcommand{\sign}{\operatorname{sign}}

\newcommand{\tick}{$\checkmark$}
\newcommand{\cross}{$\times$}

%

\newcommand{\argmin}{{\operatorname{argmin }}}
\newcommand{\argmax}{{\operatorname{argmax }}}
\newcommand{\argminUnique}[2]{\underset{#1}{\operatorname{argmin }}\, #2}
\newcommand{\argmaxUnique}[2]{\underset{#1}{\operatorname{argmax }}\, #2}

\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\E}[2]{\underset{#1}{\mathbb{E}}\left[ #2 \right]}
\newcommand{\ES}[2]{\underset{#1}{\mathbb{E}}\, #2}

%

\newcommand{\A}{\mathsf{A}}
\newcommand{\C}{\mathsf{C}}
\newcommand{\N}{\mathsf{N}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\X}{{x}}
\newcommand{\Y}{{y}}
\newcommand{\SSf}{\mathsf{S}}
\newcommand{\Z}{Z}
\newcommand{\T}{\mathbf{T}}

\newcommand{\barX}{\overline{\X}}
\newcommand{\barY}{\overline{\Y}}

%

\newcommand{\ACal}{\mathscr{A}}
\newcommand{\BCal}{\mathscr{B}}
\newcommand{\CCal}{\mathscr{C}}
\newcommand{\DCal}{\mathscr{D}}
\newcommand{\ECal}{\mathscr{E}}
\newcommand{\FCal}{\mathscr{F}}
\newcommand{\HCal}{\mathscr{H}}
\newcommand{\ICal}{\mathscr{I}}
\newcommand{\LCal}{\mathscr{L}}
\newcommand{\MCal}{\mathscr{M}}
\newcommand{\NCal}{\mathscr{N}}
\newcommand{\PCal}{\mathscr{P}}
\newcommand{\RCal}{\mathscr{R}}
\newcommand{\SCal}{\mathscr{S}}
\newcommand{\TCal}{\mathscr{T}}
\newcommand{\UCal}{\mathscr{U}}
\newcommand{\VCal}{\mathscr{V}}
\newcommand{\XCal}{\mathscr{X}}
\newcommand{\YCal}{\mathscr{Y}}
\newcommand{\ZCal}{\mathscr{Z}}

%

\newcommand{\Real}{\mathbb{R}}
\newcommand{\RealPos}{\Real_+}
\newcommand{\PMOne}{\{ \pm 1 \}}

%

\newcommand{\mathup}[1]{\text{\textup{#1}}}

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\PrZ}{\mathbb{P}}
\newcommand{\PTr}{\Pr_{\mathrm{tr}}}
\newcommand{\PTe}{\Pr_{\mathrm{te}}}

%%%
\newcommand{\tup}{\mathrm{T}}

%%% THEOREM etc.
\newtheorem{lemma}{Lemma}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{claim}[lemma]{Claim}
\newtheorem{proposition}[lemma]{Proposition}

\theoremstyle{definition}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}

\newtcbtheorem[number within=section]%
{remark_tcb} % \begin..
{Remark} % Title
{%
fonttitle=\bfseries\upshape,fontupper=\normalsize,
colframe=green!10!black,colback=green!2!white,
colbacktitle=green!20!white,coltitle=blue!75!black,
boxsep=1pt,left=2pt,right=2pt,top=1pt,bottom=1pt,
frame hidden,boxrule=1pt,
theorem style=plain} % Style - default
{rem} % label prefix; cite as ``theo:yourlabel''

%
\newtcbtheorem[number within=section]%
{assumption_tcb} % \begin..
{Assumption} % Title
{%
fonttitle=\bfseries\upshape,fontupper=\normalsize,
colframe=blue!5!black,colback=blue!2!white,
colbacktitle=blue!10!white,coltitle=blue!75!black,
boxsep=1pt,left=2pt,right=2pt,top=1pt,bottom=1pt,
frame hidden,boxrule=1pt,
theorem style=plain} % Style - default
{asm} % label prefix; cite as ``theo:yourlabel''

